Testing gravity with the two-body problem

Gravitational waves provide a new probe into the strong-field regime of gravity. It is thus essential to identify the predictions of General Relativity on the nature of the two-body problem, and to contrast them to alternative theories. This thesis aims at comparing the predictions of General Relativity and scalar-tensor theories on gravitational observables using Effective Field Theory techniques. In a first part, we show how simple scalar-tensor theories can be embedded in the Non-Relativistic General Relativity approach to the two-body problem and highlight their essential features. Furthermore, we study the effects of a disformal coupling of the scalar on the two-body dynamics and introduce a resummation technique. This new Non-Relativistic Scalar-Tensor formalism will provide a basis for the study of the Vainshtein mechanism in two-body configurations which is at the core of the second part of this thesis. Finally, in a last part we devise an Effective Field Theory formalism adapted to gravitational wave generation in theories featuring scalar hair, in the extreme mass ratio regime.

==> Chapters/Chapter1_example.tex <==
% Chapter 1

\chapter{Chapter Title Here} % Main chapter title

\label{Chapter1} % For referencing the chapter elsewhere, use \ref{Chapter1} 

%----------------------------------------------------------------------------------------

% Define some commands to keep the formatting separated from the content 
\newcommand{\keyword}[1]{\textbf{#1}}
\newcommand{\tabhead}[1]{\textbf{#1}}
\newcommand{\code}[1]{\texttt{#1}}
\newcommand{\file}[1]{\texttt{\bfseries#1}}
\newcommand{\option}[1]{\texttt{\itshape#1}}

%----------------------------------------------------------------------------------------

\section{Welcome and Thank You}
Welcome to this \LaTeX{} Thesis Template, a beautiful and easy to use template for writing a thesis using the \LaTeX{} typesetting system.

If you are writing a thesis (or will be in the future) and its subject is technical or mathematical (though it doesn't have to be), then creating it in \LaTeX{} is highly recommended as a way to make sure you can just get down to the essential writing without having to worry over formatting or wasting time arguing with your word processor.

\LaTeX{} is easily able to professionally typeset documents that run to hundreds or thousands of pages long. With simple mark-up commands, it automatically sets out the table of contents, margins, page headers and footers and keeps the formatting consistent and beautiful. One of its main strengths is the way it can easily typeset mathematics, even \emph{heavy} mathematics. Even if those equations are the most horribly twisted and most difficult mathematical problems that can only be solved on a super-computer, you can at least count on \LaTeX{} to make them look stunning.

%----------------------------------------------------------------------------------------

\section{Learning \LaTeX{}}

\LaTeX{} is not a \textsc{wysiwyg} (What You See is What You Get) program, unlike word processors such as Microsoft Word or Apple's Pages. Instead, a document written for \LaTeX{} is actually a simple, plain text file that contains \emph{no formatting}. You tell \LaTeX{} how you want the formatting in the finished document by writing in simple commands amongst the text, for example, if I want to use \emph{italic text for emphasis}, I write the \verb|\emph{text}| command and put the text I want in italics in between the curly braces. This means that \LaTeX{} is a \enquote{mark-up} language, very much like HTML.

\subsection{A (not so short) Introduction to \LaTeX{}}

If you are new to \LaTeX{}, there is a very good eBook -- freely available online as a PDF file -- called, \enquote{The Not So Short Introduction to \LaTeX{}}. The book's title is typically shortened to just \emph{lshort}. You can download the latest version (as it is occasionally updated) from here:
\url{http://www.ctan.org/tex-archive/info/lshort/english/lshort.pdf}

It is also available in several other languages. Find yours from the list on this page: \url{http://www.ctan.org/tex-archive/info/lshort/}

It is recommended to take a little time out to learn how to use \LaTeX{} by creating several, small `test' documents, or having a close look at several templates on:\\ 
\url{http://www.LaTeXTemplates.com}\\ 
Making the effort now means you're not stuck learning the system when what you \emph{really} need to be doing is writing your thesis.

\subsection{A Short Math Guide for \LaTeX{}}

If you are writing a technical or mathematical thesis, then you may want to read the document by the AMS (American Mathematical Society) called, \enquote{A Short Math Guide for \LaTeX{}}. It can be found online here:
\url{http://www.ams.org/tex/amslatex.html}
under the \enquote{Additional Documentation} section towards the bottom of the page.

\subsection{Common \LaTeX{} Math Symbols}
There are a multitude of mathematical symbols available for \LaTeX{} and it would take a great effort to learn the commands for them all. The most common ones you are likely to use are shown on this page:
\url{http://www.sunilpatel.co.uk/latex-type/latex-math-symbols/}

You can use this page as a reference or crib sheet, the symbols are rendered as large, high quality images so you can quickly find the \LaTeX{} command for the symbol you need.

\subsection{\LaTeX{} on a Mac}
 
The \LaTeX{} distribution is available for many systems including Windows, Linux and Mac OS X. The package for OS X is called MacTeX and it contains all the applications you need -- bundled together and pre-customized -- for a fully working \LaTeX{} environment and work flow.
 
MacTeX includes a custom dedicated \LaTeX{} editor called TeXShop for writing your `\file{.tex}' files and BibDesk: a program to manage your references and create your bibliography section just as easily as managing songs and creating playlists in iTunes.

%----------------------------------------------------------------------------------------

\section{Getting Started with this Template}

If you are familiar with \LaTeX{}, then you should explore the directory structure of the template and then proceed to place your own information into the \emph{THESIS INFORMATION} block of the \file{main.tex} file. You can then modify the rest of this file to your unique specifications based on your degree/university. Section \ref{FillingFile} on page \pageref{FillingFile} will help you do this. Make sure you also read section \ref{ThesisConventions} about thesis conventions to get the most out of this template.

If you are new to \LaTeX{} it is recommended that you carry on reading through the rest of the information in this document.

Before you begin using this template you should ensure that its style complies with the thesis style guidelines imposed by your institution. In most cases this template style and layout will be suitable. If it is not, it may only require a small change to bring the template in line with your institution's recommendations. These modifications will need to be done on the \file{MastersDoctoralThesis.cls} file.

\subsection{About this Template}

This \LaTeX{} Thesis Template is originally based and created around a \LaTeX{} style file created by Steve R.\ Gunn from the University of Southampton (UK), department of Electronics and Computer Science. You can find his original thesis style file at his site, here:
\url{http://www.ecs.soton.ac.uk/~srg/softwaretools/document/templates/}

Steve's \file{ecsthesis.cls} was then taken by Sunil Patel who modified it by creating a skeleton framework and folder structure to place the thesis files in. The resulting template can be found on Sunil's site here:
\url{http://www.sunilpatel.co.uk/thesis-template}

Sunil's template was made available through \url{http://www.LaTeXTemplates.com} where it was modified many times based on user requests and questions. Version 2.0 and onwards of this template represents a major modification to Sunil's template and is, in fact, hardly recognisable. The work to make version 2.0 possible was carried out by \href{mailto:vel@latextemplates.com}{Vel} and Johannes Böttcher.

%----------------------------------------------------------------------------------------

\section{What this Template Includes}

\subsection{Folders}

This template comes as a single zip file that expands out to several files and folders. The folder names are mostly self-explanatory:

\keyword{Appendices} -- this is the folder where you put the appendices. Each appendix should go into its own separate \file{.tex} file. An example and template are included in the directory.

\keyword{Chapters} -- this is the folder where you put the thesis chapters. A thesis usually has about six chapters, though there is no hard rule on this. Each chapter should go in its own separate \file{.tex} file and they can be split as:
\begin{itemize}
\item Chapter 1: Introduction to the thesis topic
\item Chapter 2: Background information and theory
\item Chapter 3: (Laboratory) experimental setup
\item Chapter 4: Details of experiment 1
\item Chapter 5: Details of experiment 2
\item Chapter 6: Discussion of the experimental results
\item Chapter 7: Conclusion and future directions
\end{itemize}
This chapter layout is specialised for the experimental sciences, your discipline may be different.

\keyword{Figures} -- this folder contains all figures for the thesis. These are the final images that will go into the thesis document.

\subsection{Files}

Included are also several files, most of them are plain text and you can see their contents in a text editor. After initial compilation, you will see that more auxiliary files are created by \LaTeX{} or BibTeX and which you don't need to delete or worry about:

\keyword{example.bib} -- this is an important file that contains all the bibliographic information and references that you will be citing in the thesis for use with BibTeX. You can write it manually, but there are reference manager programs available that will create and manage it for you. Bibliographies in \LaTeX{} are a large subject and you may need to read about BibTeX before starting with this. Many modern reference managers will allow you to export your references in BibTeX format which greatly eases the amount of work you have to do.

\keyword{MastersDoctoralThesis.cls} -- this is an important file. It is the class file that tells \LaTeX{} how to format the thesis. 

\keyword{main.pdf} -- this is your beautifully typeset thesis (in the PDF file format) created by \LaTeX{}. It is supplied in the PDF with the template and after you compile the template you should get an identical version.

\keyword{main.tex} -- this is an important file. This is the file that you tell \LaTeX{} to compile to produce your thesis as a PDF file. It contains the framework and constructs that tell \LaTeX{} how to layout the thesis. It is heavily commented so you can read exactly what each line of code does and why it is there. After you put your own information into the \emph{THESIS INFORMATION} block -- you have now started your thesis!

Files that are \emph{not} included, but are created by \LaTeX{} as auxiliary files include:

\keyword{main.aux} -- this is an auxiliary file generated by \LaTeX{}, if it is deleted \LaTeX{} simply regenerates it when you run the main \file{.tex} file.

\keyword{main.bbl} -- this is an auxiliary file generated by BibTeX, if it is deleted, BibTeX simply regenerates it when you run the \file{main.aux} file. Whereas the \file{.bib} file contains all the references you have, this \file{.bbl} file contains the references you have actually cited in the thesis and is used to build the bibliography section of the thesis.

\keyword{main.blg} -- this is an auxiliary file generated by BibTeX, if it is deleted BibTeX simply regenerates it when you run the main \file{.aux} file.

\keyword{main.lof} -- this is an auxiliary file generated by \LaTeX{}, if it is deleted \LaTeX{} simply regenerates it when you run the main \file{.tex} file. It tells \LaTeX{} how to build the \emph{List of Figures} section.

\keyword{main.log} -- this is an auxiliary file generated by \LaTeX{}, if it is deleted \LaTeX{} simply regenerates it when you run the main \file{.tex} file. It contains messages from \LaTeX{}, if you receive errors and warnings from \LaTeX{}, they will be in this \file{.log} file.

\keyword{main.lot} -- this is an auxiliary file generated by \LaTeX{}, if it is deleted \LaTeX{} simply regenerates it when you run the main \file{.tex} file. It tells \LaTeX{} how to build the \emph{List of Tables} section.

\keyword{main.out} -- this is an auxiliary file generated by \LaTeX{}, if it is deleted \LaTeX{} simply regenerates it when you run the main \file{.tex} file.

So from this long list, only the files with the \file{.bib}, \file{.cls} and \file{.tex} extensions are the most important ones. The other auxiliary files can be ignored or deleted as \LaTeX{} and BibTeX will regenerate them.

%----------------------------------------------------------------------------------------

\section{Filling in Your Information in the \file{main.tex} File}\label{FillingFile}

You will need to personalise the thesis template and make it your own by filling in your own information. This is done by editing the \file{main.tex} file in a text editor or your favourite LaTeX environment.

Open the file and scroll down to the third large block titled \emph{THESIS INFORMATION} where you can see the entries for \emph{University Name}, \emph{Department Name}, etc \ldots

Fill out the information about yourself, your group and institution. You can also insert web links, if you do, make sure you use the full URL, including the \code{http://} for this. If you don't want these to be linked, simply remove the \verb|\href{url}{name}| and only leave the name.

When you have done this, save the file and recompile \code{main.tex}. All the information you filled in should now be in the PDF, complete with web links. You can now begin your thesis proper!

%----------------------------------------------------------------------------------------

\section{The \code{main.tex} File Explained}

The \file{main.tex} file contains the structure of the thesis. There are plenty of written comments that explain what pages, sections and formatting the \LaTeX{} code is creating. Each major document element is divided into commented blocks with titles in all capitals to make it obvious what the following bit of code is doing. Initially there seems to be a lot of \LaTeX{} code, but this is all formatting, and it has all been taken care of so you don't have to do it.

Begin by checking that your information on the title page is correct. For the thesis declaration, your institution may insist on something different than the text given. If this is the case, just replace what you see with what is required in the \emph{DECLARATION PAGE} block.

Then comes a page which contains a funny quote. You can put your own, or quote your favourite scientist, author, person, and so on. Make sure to put the name of the person who you took the quote from.

Following this is the abstract page which summarises your work in a condensed way and can almost be used as a standalone document to describe what you have done. The text you write will cause the heading to move up so don't worry about running out of space.

Next come the acknowledgements. On this page, write about all the people who you wish to thank (not forgetting parents, partners and your advisor/supervisor).

The contents pages, list of figures and tables are all taken care of for you and do not need to be manually created or edited. The next set of pages are more likely to be optional and can be deleted since they are for a more technical thesis: insert a list of abbreviations you have used in the thesis, then a list of the physical constants and numbers you refer to and finally, a list of mathematical symbols used in any formulae. Making the effort to fill these tables means the reader has a one-stop place to refer to instead of searching the internet and references to try and find out what you meant by certain abbreviations or symbols.

The list of symbols is split into the Roman and Greek alphabets. Whereas the abbreviations and symbols ought to be listed in alphabetical order (and this is \emph{not} done automatically for you) the list of physical constants should be grouped into similar themes.

The next page contains a one line dedication. Who will you dedicate your thesis to?

Finally, there is the block where the chapters are included. Uncomment the lines (delete the \code{\%} character) as you write the chapters. Each chapter should be written in its own file and put into the \emph{Chapters} folder and named \file{Chapter1}, \file{Chapter2}, etc\ldots Similarly for the appendices, uncomment the lines as you need them. Each appendix should go into its own file and placed in the \emph{Appendices} folder.

After the preamble, chapters and appendices finally comes the bibliography. The bibliography style (called \option{authoryear}) is used for the bibliography and is a fully featured style that will even include links to where the referenced paper can be found online. Do not underestimate how grateful your reader will be to find that a reference to a paper is just a click away. Of course, this relies on you putting the URL information into the BibTeX file in the first place.

%----------------------------------------------------------------------------------------

\section{Thesis Features and Conventions}\label{ThesisConventions}

To get the best out of this template, there are a few conventions that you may want to follow.

One of the most important (and most difficult) things to keep track of in such a long document as a thesis is consistency. Using certain conventions and ways of doing things (such as using a Todo list) makes the job easier. Of course, all of these are optional and you can adopt your own method.

\subsection{Printing Format}

This thesis template is designed for double sided printing (i.e. content on the front and back of pages) as most theses are printed and bound this way. Switching to one sided printing is as simple as uncommenting the \option{oneside} option of the \code{documentclass} command at the top of the \file{main.tex} file. You may then wish to adjust the margins to suit specifications from your institution.

The headers for the pages contain the page number on the outer side (so it is easy to flick through to the page you want) and the chapter name on the inner side.

The text is set to 11 point by default with single line spacing, again, you can tune the text size and spacing should you want or need to using the options at the very start of \file{main.tex}. The spacing can be changed similarly by replacing the \option{singlespacing} with \option{onehalfspacing} or \option{doublespacing}.

\subsection{Using US Letter Paper}

The paper size used in the template is A4, which is the standard size in Europe. If you are using this thesis template elsewhere and particularly in the United States, then you may have to change the A4 paper size to the US Letter size. This can be done in the margins settings section in \file{main.tex}.

Due to the differences in the paper size, the resulting margins may be different to what you like or require (as it is common for institutions to dictate certain margin sizes). If this is the case, then the margin sizes can be tweaked by modifying the values in the same block as where you set the paper size. Now your document should be set up for US Letter paper size with suitable margins.

\subsection{References}

The \code{biblatex} package is used to format the bibliography and inserts references such as this one \parencite{Reference1}. The options used in the \file{main.tex} file mean that the in-text citations of references are formatted with the author(s) listed with the date of the publication. Multiple references are separated by semicolons (e.g. \parencite{Reference2, Reference1}) and references with more than three authors only show the first author with \emph{et al.} indicating there are more authors (e.g. \parencite{Reference3}). This is done automatically for you. To see how you use references, have a look at the \file{Chapter1.tex} source file. Many reference managers allow you to simply drag the reference into the document as you type.

Scientific references should come \emph{before} the punctuation mark if there is one (such as a comma or period). The same goes for footnotes\footnote{Such as this footnote, here down at the bottom of the page.}. You can change this but the most important thing is to keep the convention consistent throughout the thesis. Footnotes themselves should be full, descriptive sentences (beginning with a capital letter and ending with a full stop). The APA6 states: \enquote{Footnote numbers should be superscripted, [...], following any punctuation mark except a dash.} The Chicago manual of style states: \enquote{A note number should be placed at the end of a sentence or clause. The number follows any punctuation mark except the dash, which it precedes. It follows a closing parenthesis.}

The bibliography is typeset with references listed in alphabetical order by the first author's last name. This is similar to the APA referencing style. To see how \LaTeX{} typesets the bibliography, have a look at the very end of this document (or just click on the reference number links in in-text citations).

\subsubsection{A Note on bibtex}

The bibtex backend used in the template by default does not correctly handle unicode character encoding (i.e. "international" characters). You may see a warning about this in the compilation log and, if your references contain unicode characters, they may not show up correctly or at all. The solution to this is to use the biber backend instead of the outdated bibtex backend. This is done by finding this in \file{main.tex}: \option{backend=bibtex} and changing it to \option{backend=biber}. You will then need to delete all auxiliary BibTeX files and navigate to the template directory in your terminal (command prompt). Once there, simply type \code{biber main} and biber will compile your bibliography. You can then compile \file{main.tex} as normal and your bibliography will be updated. An alternative is to set up your LaTeX editor to compile with biber instead of bibtex, see \href{http://tex.stackexchange.com/questions/154751/biblatex-with-biber-configuring-my-editor-to-avoid-undefined-citations/}{here} for how to do this for various editors.

\subsection{Tables}

Tables are an important way of displaying your results, below is an example table which was generated with this code:

{\small
\begin{verbatim}
\begin{table}
\caption{The effects of treatments X and Y on the four groups studied.}
\label{tab:treatments}
\centering
\begin{tabular}{l l l}
\toprule
\tabhead{Groups} & \tabhead{Treatment X} & \tabhead{Treatment Y} \\
\midrule
1 & 0.2 & 0.8\\
2 & 0.17 & 0.7\\
3 & 0.24 & 0.75\\
4 & 0.68 & 0.3\\
\bottomrule\\
\end{tabular}
\end{table}
\end{verbatim}
}

\begin{table}
\caption{The effects of treatments X and Y on the four groups studied.}
\label{tab:treatments}
\centering
\begin{tabular}{l l l}
\toprule
\tabhead{Groups} & \tabhead{Treatment X} & \tabhead{Treatment Y} \\
\midrule
1 & 0.2 & 0.8\\
2 & 0.17 & 0.7\\
3 & 0.24 & 0.75\\
4 & 0.68 & 0.3\\
\bottomrule\\
\end{tabular}
\end{table}

You can reference tables with \verb|\ref{<label>}| where the label is defined within the table environment. See \file{Chapter1.tex} for an example of the label and citation (e.g. Table~\ref{tab:treatments}).

\subsection{Figures}

There will hopefully be many figures in your thesis (that should be placed in the \emph{Figures} folder). The way to insert figures into your thesis is to use a code template like this:
\begin{verbatim}
\begin{figure}
\centering
\includegraphics{Figures/Electron}
\decoRule
\caption[An Electron]{An electron (artist's impression).}
\label{fig:Electron}
\end{figure}
\end{verbatim}
Also look in the source file. Putting this code into the source file produces the picture of the electron that you can see in the figure below.

\begin{figure}[th]
\centering
\includegraphics{Figures/Electron}
\decoRule
\caption[An Electron]{An electron (artist's impression).}
\label{fig:Electron}
\end{figure}

Sometimes figures don't always appear where you write them in the source. The placement depends on how much space there is on the page for the figure. Sometimes there is not enough room to fit a figure directly where it should go (in relation to the text) and so \LaTeX{} puts it at the top of the next page. Positioning figures is the job of \LaTeX{} and so you should only worry about making them look good!

Figures usually should have captions just in case you need to refer to them (such as in Figure~\ref{fig:Electron}). The \verb|\caption| command contains two parts, the first part, inside the square brackets is the title that will appear in the \emph{List of Figures}, and so should be short. The second part in the curly brackets should contain the longer and more descriptive caption text.

The \verb|\decoRule| command is optional and simply puts an aesthetic horizontal line below the image. If you do this for one image, do it for all of them.

\LaTeX{} is capable of using images in pdf, jpg and png format.

\subsection{Typesetting mathematics}

If your thesis is going to contain heavy mathematical content, be sure that \LaTeX{} will make it look beautiful, even though it won't be able to solve the equations for you.

The \enquote{Not So Short Introduction to \LaTeX} (available on \href{http://www.ctan.org/tex-archive/info/lshort/english/lshort.pdf}{CTAN}) should tell you everything you need to know for most cases of typesetting mathematics. If you need more information, a much more thorough mathematical guide is available from the AMS called, \enquote{A Short Math Guide to \LaTeX} and can be downloaded from:
\url{ftp://ftp.ams.org/pub/tex/doc/amsmath/short-math-guide.pdf}

There are many different \LaTeX{} symbols to remember, luckily you can find the most common symbols in \href{http://ctan.org/pkg/comprehensive}{The Comprehensive \LaTeX~Symbol List}.

You can write an equation, which is automatically given an equation number by \LaTeX{} like this:
\begin{verbatim}
\begin{equation}
E = mc^{2}
\label{eqn:Einstein}
\end{equation}
\end{verbatim}

This will produce Einstein's famous energy-matter equivalence equation:
\begin{equation}
E = mc^{2}
\label{eqn:Einstein}
\end{equation}

All equations you write (which are not in the middle of paragraph text) are automatically given equation numbers by \LaTeX{}. If you don't want a particular equation numbered, use the unnumbered form:
\begin{verbatim}
\[ a^{2}=4 \]
\end{verbatim}

%----------------------------------------------------------------------------------------

\section{Sectioning and Subsectioning}

You should break your thesis up into nice, bite-sized sections and subsections. \LaTeX{} automatically builds a table of Contents by looking at all the \verb|\chapter{}|, \verb|\section{}|  and \verb|\subsection{}| commands you write in the source.

The Table of Contents should only list the sections to three (3) levels. A \verb|chapter{}| is level zero (0). A \verb|\section{}| is level one (1) and so a \verb|\subsection{}| is level two (2). In your thesis it is likely that you will even use a \verb|subsubsection{}|, which is level three (3). The depth to which the Table of Contents is formatted is set within \file{MastersDoctoralThesis.cls}. If you need this changed, you can do it in \file{main.tex}.

%----------------------------------------------------------------------------------------

\section{In Closing}

You have reached the end of this mini-guide. You can now rename or overwrite this pdf file and begin writing your own \file{Chapter1.tex} and the rest of your thesis. The easy work of setting up the structure and framework has been taken care of for you. It's now your job to fill it out!

Good luck and have lots of fun!

\begin{flushright}
Guide written by ---\\
Sunil Patel: \href{http://www.sunilpatel.co.uk}{www.sunilpatel.co.uk}\\
Vel: \href{http://www.LaTeXTemplates.com}{LaTeXTemplates.com}
\end{flushright}


==> Chapters/Chapter8.tex <==
\chapter{A three body system in the cubic Galileon} \label{Chapter8}

%TODO : refs on three bodies... And say we can also apply to EMRI
%TODO : check that cubic gal is not constrained by filippo

In the last Chapter we have solved for the Earth-Moon motion in a theory with Vainshtein screening by assuming that the Sun acts only as a background field so that superposition principle holds in the sense that the Earth-Moon two-body energy can be calculated by ignoring the Sun. This assumption was valid under the following distance hierarchy,
\begin{equation}
\frac{r_\mathrm{EM}}{r_{*, E}} \ll \frac{r_\mathrm{ES}}{r_{*,S}} \; ,
\end{equation}
where $r_\mathrm{EM}$ is the Earth-Moon distance, $r_\mathrm{ES}$ the Earth-Sun distance, $r_{*, E}$ the Vainshtein radius of the Earth and $r_{*, S}$ the Vainshtein radius of the Sun. In this Chapter, we will consider the opposite situation, in which the distance between the two small bodies is large; the system which we will consider is composed of three Black Holes (BH), a supermassive one (the 'Sun') and two solar-size ones (the 'Earth' and the 'Moon'). Supermassive BH typically lie at the center of galaxies; the inspiral of solar-size BH around supermassive ones is expected to produce GW detectable by the future space-borne interferometer LISA (see Section~\ref{subsec:current_planned_inter}), and can lead to an interesting phenomenology such as Kozai-Lidov oscillations~\cite{Randall:2019sab,Randall:2017jop,Randall:2018nud}. Such a system could thus allow for a perturbative treatment (the small BH move in the background field generated by the supermassive one) and is observationally relevant, which makes it very interesting as a probe of the Vainshtein mechanism.

For definiteness, we will consider a cubic Galileon theory which is known from Section~\ref{subsec:Galileons} to exhibit the Vainshtein screening mechanism, so that the total action of our system is
\begin{equation} \label{eq:base_action}
S = \frac{1}{2} \int \mathrm{d}^4 x \sqrt{-g} \left[ \mpl^2 R - (\partial \varphi)^2 - \frac{1}{\Lambda^3} (\partial \varphi)^2 \square \varphi \right] + S_m[\tilde g_{\mu \nu}, \psi_i] \; ,
\end{equation}
where $\Lambda$ is the energy scale of the cubic Galileon interaction, and in this Chapter we denote the scalar by $\varphi$ to avoid confusion with the angular variable $\phi$. In order to give a rough estimate for the latter, if the Galileon is supposed to contribute to the accelerated expansion of our universe one should impose $\Lambda^3 \sim H^2 \mpl$. Nevertheless, we will keep this scale arbitrary and assume that a cosmological constant lies behind the acceleration. The metric $\tilde g_{\mu \nu}$ is as usual the Jordan frame metric, which couples to matter. We take it to be simply conformally related to the Einstein frame metric, $\tilde g_{\mu \nu} = A^2(\varphi) g_{\mu \nu}$ where $A(\varphi) = e^{\beta \varphi / \mpl}$ is the universal coupling factor (we will se below that contrary to BDT theories, the cubic Galileon predicts a dipolar power even considering the scalar charge to be universal).

We have seen in Section~\ref{sec:tests_GW} that the cubic Galileon does not change the speed of gravity and so it is not constrained by the GW speed bound (this bound essentially removes any quartic or quintic Galileon of any cosmological model). However, the instability bound mentioned in the same Section~\ref{sec:tests_GW} indeed applies to the cubic Galileon, and this severely limits its cosmological significance (this is confirmed by other cosmological constraints~\cite{Bellini_2013}); furthermore,
 as we have seen in the introduction of the last Chapter, the perihelion constraint provides a relevant bound on the size of a cubic Galileon operator. In this Chapter, we will analyze independently which kind of constraints we can obtain on the cubic Galileon from GW emitted by the triple system which we consider. We will carry out our computations independently of the fact that the cubic Galileon participates in dark energy (in other words, we will keep the energy scale $\Lambda$ introduced below in Eq. \eqref{eq:base_action} arbitrary, although we will assume a cosmological scaling in most of the order-of-magnitude estimates). 
 

As a  phenomenological test of the existence of scalar fields, BHs usually do not present many features and are deemed to be  irrelevant probes because of the no-hair theorem which forbids the appearance of any scalar profile around BH. Chapter~\ref{Chapter9} will be entirely dedicated to no-hair theorems, so let us simply state here that
 there are many ways out of this restriction. Indeed the  time-dependence of a scalar field at spatial infinity induces scalar hair around BHs~\cite{Jacobson_1999}. This time-dependence could be due to cosmological boundary conditions or to the environment in which the BHs are located~\cite{Horbatsch_2012}. Concerning the Galileon, we will review in the next Chapter, Section~\ref{sec:BH_hair_timedep}, how hair can be  induced by an asymptotic timelike gradient of the scalar, showing that it can even lead to the generation of large scalar couplings. For the moment though, all what we need to know is that BH couple to the scalar with an \textit{effective} coupling $\beta_\mathrm{eff}$ which is a free parameter of our problem.
 
 
Even if one circumvents the no-hair theorem, the modification of the GW signal of inspiralling binaries by the Galileon field has been shown to be screened by the Vainshtein mechanism even in this very dynamical situation~\cite{deRham:2012fg,dar_scalar_2018,deRham:2012fw}, which makes any deviation from GR very suppressed despite the fact that scalar-tensor theories generically predict dipole radiation which is enhanced with respect to the quadrupole in the post-Newtonian expansion (see Chapter~\ref{Chapter4}). However, GW detectors such as LISA can monitor the inspiral of compact objects during a large number of GW cycles, thereby greatly enhancing the potentiality of detecting any deviation from GR. It is thus worth investigating  the detectability of a Galileon field by LISA.

Before giving more  details of our calculations, let us present a few order-of-magnitude estimates characteristic of  our system. We will consider a massive BH of mass $m_0 \sim 10^6 M_\odot$ at the centre of a galaxy, and two 'small' BHs of mass $m_1, m_2 \sim 30 M_\odot$ orbiting in its vicinity. For simplicity, all trajectories are assumed to be circular, i.e the two BHs are in a circular orbit of radius $d$ and their common barycentre is in circular orbit of radius $r$ around the massive BH, with $d \lesssim r$. A more realistic treatment would necessitate to take  into account the eccentricity of the orbits which can grow to significant values in this kind of configurations~\cite{Randall:2019sab,Randall:2017jop,Randall:2018nud}. Figure~\ref{fig:physical_situation} provides a schematic representation of the system which we consider.


\begin{figure}[h!]
\center \includegraphics[width=.6\columnwidth]{Figures/physical_situation.pdf}
\caption[Schematic representation of the length-scales of the problem at stake]{Schematic representation of the length-scales of the problem at stake. The distances have to satisfy eqs. \eqref{eq:condition_green}, and $\hat n$ is the normal to the plane of rotation of the binary system formed by the two small BHs}
\label{fig:physical_situation}
\end{figure}

 At a frequency of approximately $\omega = 10^{-3}$ Hz and higher, the two BHs could emit gravitational waves potentially detectable in the LISA band provided that their amplitude is large enough. This frequency corresponds to a maximal separation of the binary system  of  $d_\mathrm{max} = (Gm_1/\omega^2)^{1/3} \sim 10^9$ m $\sim 0.01$ AU, using Kepler's third law. Higher frequencies lead to shorter distances. On the other hand, we will see in Section~\ref{sec:setup_chap8} that in order for our perturbative calculation to be valid, one should require $d \gtrsim r/50$ so that the binary system should be closer than $0.5$ AU from the central black hole. The corresponding Vainshtein suppression of the fifth force is $(r/r_*)^{3/2} \sim 10^{-16}$ where $r_*$ is the Vainshtein radius.
 
  Despite this strong suppression, we will show that the Galileon field can lead to observable changes in the GW phase provided one chooses moderately large values for the effective scalar coupling.
 We then compute both the two-body energy and the power dissipated from the system. While the former involves the usual Vainshtein suppression and leads to negligible departures from GR, the latter contains non-trivial powers of the lengthscales of the system which makes it non-negligible in this particular configuration. We finally derive the modification of the binary dynamics when the scalar power is subdominant, and show that it could be observable thanks to the large number of gravitational wave cycles.
 Our final and most important results are Eqs. \eqref{eq:delta_phi_EMRI}~-~\eqref{eq:delta_phi_binary} concerning the contribution of the Galileon operator to the total GW phase. Part of ours results (and in particular Eq. \eqref{eq:delta_phi_EMRI}) will also be valid for a system of a single solar-size BH orbiting a supermassive one, and will provide a useful cross-check of our computations since this case has already been considered in Ref.~\cite{deRham:2012fw}. 
%This type of events should be much more common than the three-body case we 









\section{Perturbative treatment of the interactions} \label{sec:setup_chap8}

Emission of gravitational and scalar waves by a system of binary pulsars in the presence of Galileon interactions has been studied in Refs.~\cite{deRham:2012fg,deRham:2012fw,dar_scalar_2018}. In this Chapter, we will consider a different physical situation amenable to a perturbative treatment.
The system we will study is a three-body system, which is composed of a massive BH of mass $\mathcal{O}(10^6) M_\odot$ at the origin of the coordinates, and two 'small' BHs of mass $\mathcal{O}(10) M_\odot$. We will generically denote distances to the massive BH  by $r$, and distances between the small BHs by $d$. 


 In the following Subsection, we will parametrize the three-body problem, after what we will show how one can solve for the conservative and dissipative dynamics of the system by a perturbative treatment of the Vainshtein interactions.

\subsection{Three-body BHs: parametrisation of the problem} \label{subsec:param}


We are interested in the system of three BHs as described in the introduction and will assume that the  BHs are described by a point-particle action.
For simplicity, we will assume all the motions to be circular, i.e the two small BHs are in a circular orbit of frequency $\Omega$ around their common barycentre. We call this motion the 'inner orbit', which is itself in circular orbit of frequency $\Omega_0$ around the massive BH. We call its motion the 'outer orbit'. This has been schematically illustrated in figure~\ref{fig:physical_situation}. A more realistic treatment would necessitate to take  into account the eccentricity of the orbits which can grow to significant values in this kind of configurations~\cite{Randall:2019sab,Randall:2017jop,Randall:2018nud}.

We perform the analysis in the frame co-rotating with the centre-of-mass of the binary. Denoting by $\vec d = \vec x_1 - \vec x_2$ and $\vec r$ the position of the centre-of-mass of the binary, we get
\begin{equation}
\vec x_1 \equiv \vec r + \vec d_1 = \vec r + (1-X) \vec d, \quad \vec x_2 \equiv \vec r + \vec d_2 = \vec r - X \vec d
\end{equation}
where $X = m_1/(m_1+m_2)$. The $z$ axis of the coordinate system is chosen to point from the distant massive object of mass $m_0$ at the origin to the centre-of-mass $\vec r$.

The orientation of the axis of rotation of the system is arbitrary and we choose to parametrise it with Euler angles $\hat a$, $\hat b$ and $\hat c$. This means that $\vec d$ is written as
\begin{equation}
\vec d = R_z(\hat c) R_x(\hat b) R_z(\hat a) (d \cos(\Omega t), d \sin(\Omega t), 0)^T \; ,
\end{equation}
where the $R_i$'s are rotation matrices around the $i$ axis. However, since the orientation of the $x$ and $y$ axes is defined up to an arbitrary rotation, we can fix $\hat c = 0$. In explicit coordinates $\vec d$ reads
\begin{equation}
\vec d = d
\begin{cases} \cos(\Omega t + \hat a) \\
  \cos\hat b \sin(\Omega t + \hat a) \\
  \sin\hat b \sin(\Omega t + \hat a)

\end{cases} \; ,
\end{equation}
which shows that $\hat a$ can be absorbed into a redefinition of the origin of time, so we set $\hat a = 0$ from now on.

Then the distance of object $1$ to the massive object $0$ is
\begin{equation}
\vert \vec x_1 \vert^2 = r^2 + 2 r d_1 \sin\hat b \sin(\Omega t) + d_1^2 \; ,
\end{equation}
where we recall that $r$ is the distance of the centre-of-mass to the massive object. The equations are the same for the object $2$ by just replacing $d_1$ by $d_2$.





\subsection{Redressing the interactions} \label{sec:three_body_problem}



 In this subsection, we will show that there is a regime where one can perturbatively calculate the cubic Galileon corrections to the orbital parameters of the binary system, giving rise to a modification of the dynamics detectable in a GW signal. The rest of the Chapter will be devoted to the exact calculation of this correction and its phenomenological implications. The derivation that we will present here closely follows the one which we presented in the last Chapter, Section~\ref{sec:three-body}, except that we will be interested in the opposite regime where the two small objects are far apart.

%TODO : replace pi by phi

We take the matter action in Eq. \eqref{eq:base_action} to be constituted of three sources with masses $m_0$, $m_1$ and $m_2$. In this subsection we will concentrate on the scalar part of the action for illustrative purposes. On flat spacetime and expanding to first order in $\varphi / \mpl$, the scalar part of the matter action is
\begin{equation} \label{eq:matter_action_eff}
S_m = \int d^4 x \; \beta_\mathrm{eff} \frac{\varphi}{\mpl} T \; ,
\end{equation}
where we recall that $\beta_\mathrm{eff}$ is the effective scalar coupling to BH (see next Chapter, Section~\ref{sec:evading_no_hair}), and the three bodies contribute as
\begin{equation}
T = - m_0 \delta^3(\vec{x}) - m_1 \delta^3(\vec{x} - \vec{x}_1)- m_2 \delta^3(\vec{x} - \vec{x}_2) \; ,
\end{equation}
up to relativistic corrections. Since $m_0 \ll m_1,m_2$, let us first consider the field $\phi_0$ generated by the central BH only. In fact, we already gave this field in Section~\ref{subsec:Galileons} when explaining the basics of the Vainshtein mechanism. Taking into account the supplementary factor of $\beta_\mathrm{eff}$ compared to Section~\ref{subsec:Galileons}, in the screened regime the field is given by
\begin{equation}
\label{eq:phi_SS}
\varphi_0' =  \left( \frac{\beta_\mathrm{eff} m_0 \Lambda^3 }{8 \pi \mpl r} \right)^{1/2}
 =  \frac{\beta_\mathrm{eff} m_0}{8 \pi \mpl r_{V,0}^2} \left( \frac{r_{V,0}}{r} \right)^{1/2} \;,  \quad r_{V,0}^3 = \frac{\beta_\mathrm{eff} m_0}{8 \pi \mpl \Lambda^3} \; .
\end{equation}

Let us now take into account the small perturbations created by the masses $m_1, m_2$
by writing the field decomposition $\phi = \phi_0 + \psi$, where $\psi$ represents a fluctuation of the scalar field generated by the two small BHs. In terms of this variable, the action reads 
\begin{align} \label{eq:action_expanded}
\begin{split}
S[\varphi] &= S[\varphi_0] + \int d^4 x \left( -\frac{1}{2} (\partial \psi)^2 - \frac{1}{2\Lambda^3} \left[ (\partial\psi)^2 \Box \varphi_0 + 2 \partial_\mu \psi \partial^\mu \varphi_0 \Box \psi \right] \right. \\
 &- \left. \frac{1}{2\Lambda^3} (\partial\psi)^2 \Box \psi  + \frac{\beta_\mathrm{eff}}{\mpl} \psi \tilde{T} \right) \; ,
\end{split}
\end{align}
where we have eliminated the linear terms with the equations of motion and introduced $\tilde T$ as
\begin{equation} \label{eq:tilde_T}
\tilde{T} = - m_1 \delta^3(\vec{x} - \vec{x}_1)- m_2 \delta^3(\vec{x} - \vec{x}_2) \; .
\end{equation}
By definition, the Vainshtein regime in the background of the central BH occurs  when the Galileon terms dominate the quadratic term $(\partial \psi)^2$ in the action. The behaviour of $\psi$ depends on which Galileonic term dominates in the action. In the last Chapter, we were interested in the case where the term cubic in $\psi$ (in the second line of Eq. \eqref{eq:action_expanded}) dominates the action. Let us rather assume here that the quadratic term dominates and derive the confition under which this statement is valid. We can canonically normalize $\psi$ by the following (order-of-magnitude) field redefinition:
\begin{equation}
\tilde \psi = \sqrt{Z} \psi \; , \quad Z = \frac{\square \varphi_0}{\Lambda^3} \sim \left( \frac{r_{V,0}}{r} \right)^{3/2}
\end{equation}
This has the effect of suppressing the scalar coupling in the canonically normalized theory,
\begin{equation}
\tilde \beta_\mathrm{eff} = \frac{\beta_\mathrm{eff}}{\sqrt{Z}} \; .
\end{equation}
The theory is then a simple BDT theory with scalar coupling $\tilde \beta_\mathrm{eff}$.
Solving for the field $\tilde \psi$ generated by (say) the first particle gives
\begin{equation}
\tilde \psi \sim \frac{\tilde \beta_\mathrm{eff} m_1}{\mpl d} \; ,
\end{equation}
where $d$ is the distance to the first particle. Then, the ratio of the cubic term in the action \eqref{eq:action_expanded} to the quadratic term is
\begin{equation}
\frac{(\partial \psi)^2 \Box \psi}{(\partial \psi)^2 \Box \varphi_0} \sim \frac{\Box \psi}{\Box \varphi_0} \sim \left( \frac{r^3 m_1}{d^3 m_0} \right)^{1/2} \; ,
\end{equation}
where we have used the scaling $\Box \varphi_0 \sim \varphi_0 / r^2$, $\Box \psi \sim \psi / d^2$.
This means that,
 if the distance between the light bodies is large enough, i.e
\begin{equation} \label{eq:condition_green}
\frac{d}{r_{V,1}} \sim \frac{d}{r_{V,2}}  \gtrsim \frac{r}{r_{V,0}}
\end{equation}
then the dominant term for $\psi$ in the action is the quadratic one. In the last equation, we have denoted by $r_{V,1}$ the Vainshtein radius \eqref{eq:phi_SS} of the small mass $m_1$, and similarly for $m_2$.  We will place ourselves in this physical situation. This can also be interpreted as the two BH's being outside their respective 'redressed' Vainshtein radius defined by
\begin{equation}
\tilde r_{V,\alpha}^3= \frac{\tilde \beta_\mathrm{eff} m_\alpha}{8 \pi \mpl \tilde\Lambda^3}, \ \alpha=1,2  \; .
\end{equation}
In this equation, the redressed energy scale also arise from canonically normalising the fluctuation $\psi$ and is of the form $\tilde \Lambda= \sqrt Z \Lambda $.
The condition $d \gtrsim  \tilde r_{V,1}$ expressing the fact the the two BHs should be outside their redressed Vainshtein radius is perfectly equivalent to the condition \eqref{eq:condition_green}.

If the small objects masses are taken to be of the order of ten solar masses, while the central object is a supermassive BH with $m_0 \sim 10^6 M_\odot$, then the condition \eqref{eq:condition_green} translates into
\begin{equation}
d \gtrsim \frac{r}{50}\;.
\end{equation}
Hence, this condition enables us to calculate the cubic Galileon corrections to the orbital parameters  perturbatively.



Before moving on, it is worth noting that the Vainshtein condition \eqref{eq:condition_green} on the distances exactly imposes $\Omega_0 \gtrsim \Omega$. Indeed, with Kepler's law one can write
\begin{equation}
\Omega_0^2 = \frac{Gm_0}{r^3} \gtrsim \frac{Gm_i}{d^3} \simeq \Omega^2\;
\end{equation}
implying that the binary system has a rotation rate around the central BH which is larger than its own one.
%This regime starts when the two BHs are such that $\Omega\simeq \Omega_0$ initially. 


\section{Galileon propagation: the Green's function} \label{sec:Green}
In this section we exactly compute the propagation of the Galileon in the geometrical  background configuration, following the order-of-magnitude estimates of the previous subsection. For this purpose we essentially need to compute the Green's function of the second order action in perturbations. This will enable us to compute the two-body energy and the power dissipated in scalar radiation.

Let us start from our base action \eqref{eq:base_action} and split the fields according to $g_{\mu \nu} = \eta_{\mu \nu} + h_{\mu \nu}$, $\varphi = \varphi_0 + \psi$ where $\varphi_0$ is given by eq. \eqref{eq:phi_SS}. We do not consider the interactions between the scalar and the graviton since they will give subleading corrections to our results as we will argue below. This means that the action \eqref{eq:base_action} splits into the usual Einstein-Hilbert action and a cubic Galileon in flat spacetime coupled to matter through eq. \eqref{eq:matter_action_eff}. We now concentrate on the scalar part of the action, and as observed in Section~\ref{sec:three_body_problem} we keep only terms quadratic in $\psi$ to obtain
\begin{equation}
S[\varphi] = S[\varphi_0] + \int d^4 x \left(  - \frac{1}{2\Lambda^3} \left[ (\partial\psi)^2 \Box \varphi_0 + 2 \partial_\mu \psi \partial^\mu \varphi_0 \Box \psi \right]   + \frac{\beta_\mathrm{eff}}{\mpl} \psi \tilde{T} \right) \; ,
\end{equation}
where $\tilde{T}$ is given in eq. \eqref{eq:tilde_T}.

We rewrite the quadratic action for $\psi$ in spherical coordinates and integrate by parts in order to eliminate the higher derivatives on $\psi$. We find
\begin{equation}
S = S[\varphi_0] + \int d^4x \frac{1}{2} \left[ K_{t} (\partial_t \psi)^2 - K_{r} (\partial_r \psi)^2 - K_{\Omega} (\partial_\Omega \psi)^2 \right] + \frac{\beta_\mathrm{eff}}{\mpl} \psi \tilde{T}
\end{equation}
where the kinetic, angular and radial factors read
\begin{align}
K_t = 3 \left( \frac{r_*}{r} \right)^{3/2}, \qquad
K_r = 4 \left( \frac{r_*}{r} \right)^{3/2} \qquad \text{and} \qquad
K_\Omega = \left( \frac{r_*}{r} \right)^{3/2}
\end{align}
and the radius $r_*$
\begin{equation}
r_* = r_{V,0} = \left(\frac{\beta_\mathrm{eff} m_0}{8 \pi \mpl \Lambda^3} \right)^{1/3}
\end{equation}
denotes the Vainshtein radius associated to the central mass.

In order to find the two-body energy and the power dissipated in scalar radiation, we have to find the Green's function associated to this quadratic operator. It is defined by
\begin{equation}
\left[- K_t(r) \partial_t^2 + \frac{1}{r^2} \partial_r \left(r^2 K_r \partial_r \right) + \frac{K_\Omega}{r^2} \nabla_\Omega^2 \right] G(x, x') = \delta^4(x - x')
\end{equation}
where $\nabla_\Omega^2 = \partial_\theta^2 + 1/\sin^2 \theta \partial_\phi^2$. It is worth mentioning  the following special boundary condition. We will take the field to vanish at the origin of coordinates where the massive object lies. Since the field goes as $r^{1/2}$ at the origin, this is consistent, contrary to the Newtonian problem where the field goes as $1/r$ but vanishes at infinity. We can obtain the field as
\begin{equation} \label{eq:field_green_fct}
\psi(x) = \int d^4x' G(x, x') \left( - \frac{\beta_\mathrm{eff} T(x')}{\mpl} \right)
\end{equation}

In the static case, by substituting  the field in the quadratic action, we can obtain the two-body energy, defined as $\int dt E = - \Re(S_\mathrm{cl})$
\begin{equation} \label{eq:energy_green_fct}
- \Re(S_\mathrm{cl})=\int dt E = \frac{1}{2} \int d^4x d^4x' G(x, x') \frac{\beta_\mathrm{eff} T(x)}{\mpl} \frac{\beta_\mathrm{eff} T(x')}{\mpl} \; .
\end{equation}
We will follow  Refs.~\cite{andrews_galileon_2013,deRham:2012fg,chu_retarded_2013} in order to calculate the Green's function.
For static configurations, we will subtract an infinite term from the Green's function which is space-independent and does not contribute to the energy as the supports of the
matter distributions do not intersect.

 By introducing the rescaled variable $\vec u = \frac{\vec r}{r_*}$, we rewrite the previous equation as
\begin{equation}
\left( -3 r_*^2 \partial_t^2 + 4 \partial_u^2 + \frac{2}{u} \partial_u + \frac{\nabla_\Omega^2}{u^2} \right) G(\vec u, t ; \vec u', t') = \frac{\delta^3(\vec u - \vec u') \delta(t-t')}{r_*}\;.
\end{equation}
We further decompose the Green function in a Fourier and spherical harmonics basis as
\begin{equation} \label{eq:green_fourier}
G(\vec u, t ; \vec u', t') = \int \frac{d\omega}{2\pi} e^{-i \omega (t-t')} \sum_{l=0}^{\infty} R_{lm \omega}(u, u') \sum_{m=-l}^l Y_l^m[\theta, \phi] \bar Y_l^m[\theta', \phi']\;.
\end{equation}
Using the resolution of the identity
\begin{equation}
\sum_{l,m} Y_l^m[\theta, \phi] \bar Y_l^m[\theta', \phi'] = \delta( \cos(\theta) - \cos(\theta') ) \delta(\phi - \phi')
\end{equation}
one easily finds the equation for the mode function $R_{lm}$
\begin{equation} \label{eq:diffeq_R}
\left( \partial_u^2 + \frac{1}{2u} \partial_u + \frac{3}{4} \tilde \omega^2 - \frac{l(l+1)}{4 u^2} \right) R_{lm \omega}(u,u') = \frac{\delta(u - u')}{4 r_* \sqrt{u}}
\end{equation}
where $\tilde \omega = r_* \omega$.

The general continuous solution of eq. \eqref{eq:diffeq_R} is
\begin{equation}
R(u,u') = A R^1(u) R^1(u') + B R^2(u) R^2(u') + C R^1(u_<) R^2(u_>) + D R^1(u_>) R^2(u_<)
\end{equation}
where we have omitted the index $l,m, \omega$ for clarity and the constants $A,B,C,D$ are to be fixed by the normalization of the mode functions and the boundary conditions. Here we have introduced the notation $u_> = \mathrm{max}(u, u')$ and $u_< = \mathrm{min}(u, u')$, and the homogeneous solutions are given by the Bessel functions
\begin{align}
\begin{split}
R^1(u) &= \mathcal{N} u^{1/4} J_\nu \left(\sqrt{\frac{3}{4}} u \tilde \omega \right) \\
R^2(u) &= \mathcal{N} u^{1/4} J_{-\nu}\left(\sqrt{\frac{3}{4}} u \tilde \omega \right)\;,
\end{split}
\end{align}
where $\mathcal{N}$ is a normalization constant and $\nu = (2l+1)/4$. Integrating eq. \eqref{eq:diffeq_R} for $u$ close to $u'$, we get
\begin{equation}
(D-C)W = \frac{1}{4r_* \sqrt{u}}
\end{equation}
where
\begin{equation}
W = R^{1'} R^2 - R^1 R^{2'} = \frac{2 \mathcal{N}^2 \sin(\nu \pi)}{\pi \sqrt{u}}
\end{equation}
is the Wronskian of the two homogeneous solutions. We choose
\begin{equation}
\mathcal{N} = \sqrt{\frac{\pi}{8r_* \sin(\nu \pi)}}
\end{equation}
such that $D-C = 1$.

We next determine the constants from the boundary conditions. We require the flux to be purely outgoing at infinity, which corresponds to taking the retarded Green's function. On the other hand, the boundary condition at the origin can be fixed by the following observation. Consider the field produced by a variation $m \rightarrow m + \delta m$ of the central mass. From eq. \eqref{eq:phi_SS} (with a field vanishing at the origin), it is
\begin{equation}
\delta \pi_0(r) = \frac{\beta \delta m}{8\pi \mpl r_*} \left( \frac{r}{r_*} \right)^{1/2}
\end{equation}
On the other hand, from eq. \eqref{eq:field_green_fct}, we have
\begin{align}
\begin{split}
\delta \pi_0(t, \vec x) &= - \frac{\beta}{\mpl} \int d^4x' G( x, x') T( x') \\
&= \frac{\beta \delta m}{\mpl} \int dt' G(\vec r, t ; \vec 0, t')\;.
\end{split}
\end{align}
By equating these two equations, we find the boundary condition at the origin
\begin{equation}\label{eq:BC_origin}
\mathrm{lim}_{\omega \rightarrow 0} \sum_l \frac{2l+1}{4\pi} P_l(\cos(\theta)) R_{lm\omega}(u,0) = \frac{\sqrt{u}}{8\pi r_*}\;,
\end{equation}
where $P_l$ represent the Legendre polynomials, and we have used the following identities
\begin{equation}
Y_l^m(0,\phi) = \sqrt{\frac{2l+1}{4\pi}} \delta_{m0} \; , \quad Y_l^0(\theta, \phi) = \sqrt{\frac{2l+1}{4\pi}} P_l(\cos(\theta))\;.
\end{equation}

Let us examine the asymptotic behaviour for $l>0$ first. From the behaviour of the Bessel's functions at the origin
\begin{equation}
J_\nu(z) \sim \frac{1}{\Gamma(\nu+1)} \left( \frac{z}{2} \right)^\nu
\end{equation}
we immediately deduce that $B=D=0$ for $l \geq 1$ in order for the Green's function to be continuous at the origin. The solution is now
\begin{equation}
R(u,u') = A R^1(u) R^1(u') - R^1(u_<) R^2(u_>)\;.
\end{equation}
The constant $A$ is fixed by requiring the flux to be outgoing at infinity. Indeed, by rewriting the Bessel functions in terms of the two Hankel functions
\begin{align}
\begin{split}
J_\nu &= \frac{H_\nu^{(1)} +H_\nu^{(2)} }{2} \\
J_{-\nu} &= \frac{1}{2} \left( H_\nu^{(1)}(1-i \tan(\nu \pi)) - H_\nu^{(2)}(1+i \tan(\nu \pi)) \right)
\end{split}
\end{align}
and using the asymptotic behaviour at infinity
\begin{align} \label{eq:asymptotic_bessel}
\begin{split}
H_\nu^{(1)}(z) &\sim \sqrt{\frac{2}{\pi z}} e^{i\left(z-\nu \frac{\pi}{2} - \frac{\pi}{4} \right)} \\
H_\nu^{(2)}(z) &\sim \sqrt{\frac{2}{\pi z}} e^{-i\left(z-\nu \frac{\pi}{2} - \frac{\pi}{4} \right)}
\end{split}
\end{align}
the condition that the flux is purely outgoing imposes
\begin{equation}
A = - (1+i \tan(\nu \pi))
\end{equation}

Let us now examine the $l=0$ case. In this case, $R^2$ is not divergent any more at the origin but takes a finite value,
\begin{equation}
R^2(0) = \frac{1}{\Gamma(3/4)} \left( \frac{1}{8 \sqrt{3} \tilde \omega} \right)^{1/4} \sqrt{\frac{\pi}{r_*}}\;.
\end{equation}
The solution when one of the points is taken to be the origin is
\begin{equation}
R(u,0) = R^2(0) \left( B R^2(u) + D R^1(u) \right)\;.
\end{equation}
We can now use eq. \eqref{eq:BC_origin} by noticing that $R_{lm \omega}(u,0) = 0$ for $l > 0$, which gives
\begin{equation}
\mathrm{lim}_{\omega \rightarrow 0} R(u,0) = \frac{\sqrt{u}}{2 r_*}\;.
\end{equation}
This imposes $D = 1$ (so $C=0$). The $B$ coefficient multiplies a power-law divergent term which we simply subtract as it does not depend on the variables $u, u'$.  $B$ is  left undetermined here.
To find $A$ and $B$, let us rewrite the solution when one of the endpoints is taken to infinity, say $u'$,
\begin{equation}
R(u,u') = A R^1(u) R^1(u') + R^2(u)(B R^2(u') + R^1(u')) \; ,
\end{equation}
so that in order to have a purely outgoing flux, one should impose
\begin{align}
\begin{split}
A &= 0 \\
B &= \frac{1}{1+i}\;.
\end{split}
\end{align}
In conclusion, the mode functions are
\begin{equation} \label{eq:mode_functions}
\begin{array}{rclc}
R(u,u') &=& R^1(u_>) R^2(u_<) + \frac{1}{1+i} R^2(u) R^2(u') & \text{for }l=0 \\
& & & \\
R(u,u') &=& - R^1(u_<) R^2(u_>) - (1+i \tan(\nu \pi)) R^1(u) R^1(u') & \text{for }l>0  \;.
\end{array}
\end{equation}
In this way the Green's function \eqref{eq:green_fourier} is completely characterised.

\section{Static limit: $\omega \rightarrow 0$} \label{sec:static}

\subsection{The two-body energy}
Next, we shall discuss the static limit (i.e, the limit $\omega \rightarrow 0$) of the Green's function which will give rise to the two-body scalar energy. Let us focus on $l>0$ first. Then it is easy to see that the only nonzero part of $R$ is
\begin{align}
\begin{split}
R(u,u') &= - R^1(u_<) R^2(u_>) \\
&= - \frac{1}{2 (2l+1) r_*} u_<^{(l+1)/2} u_>^{-l/2}\;,
\end{split}
\end{align}
which gives upon using eq. \eqref{eq:green_fourier} and a choice of axis for $ \vec u '$ such that $\theta ' = 0$
\begin{equation}
\int dt' G(\vec u, t ; \vec u', t') \supset \frac{1}{8 \pi r_*} \left( u_<^{1/2} - \frac{u^{1/2} u'^{1/2}}{\vert \sqrt{u} \hat u - \sqrt{u'} \hat u' \vert} \right) \; ,
\end{equation}
where $\hat u = \vec{u} / u$, and we have used the Legendre polynomial identity
\begin{equation}
\frac{1}{\vert \vec x - \vec x' \vert} = \sum_{l=0}^{\infty} \frac{x'^l}{x^{l+1}} P_l(\cos\theta) \; ,
\end{equation}
where $x = \vert \vec x \vert$, $x' = \vert \vec x' \vert$ and $\theta$ is the angle between $\vec x$ and $\vec x'$.
Ignoring the divergent $R^2 R^2$ contribution as before, the $l=0$ term is similarly obtained and one finally gets for the static Green's function
\begin{equation}
\int dt' G(\vec u, t ; \vec u', t') = \frac{1}{8 \pi r_*} \left( - \frac{\rho \rho'}{\vert \vec{\rho} - \vec{\rho}' \vert}  + \rho + \rho' \right)
\end{equation}
where $\vec \rho = \sqrt{u} \hat u$.

We shall use this Green's function to find the energy. There are two types of terms in eq. \eqref{eq:energy_green_fct}: the self-energy terms and the $1-2$ interaction term. We will ignore the self-energies since these terms contribute only when finite-size effects are taken into account. In any case the evaluation of the Green's function at coincident points is not well defined because eq. \eqref{eq:condition_green} is not satisfied.
The interaction term gives the energy
\begin{equation} \label{eq:energy}
E = \frac{\beta_\mathrm{eff}^2 m_1 m_2}{2 \pi \mpl^2 r_*} \left( \rho_1 + \rho_2 - \frac{\rho_1 \rho_2}{\vert \vec{\rho}_1 - \vec{\rho}_2 \vert} \right)
\end{equation}

Let us now come back to Figure~\ref{fig:physical_situation} and give some order-of-magnitude estimates. If $d \lesssim  r$, the last term in the energy dominates
\begin{equation}
\frac{\rho_1 \rho_2}{\vert \vec{\rho}_1 - \vec{\rho}_2 \vert} \sim \sqrt{\frac{r}{r_*}} \frac{r}{d}\;.
\end{equation}
Then the ratio of this energy to the Newtonian energy $E_N \sim m_1 m_2/( \mpl^2 d)$ is
\begin{equation}
\frac{E}{E_N} \sim \beta_\mathrm{eff}^2 \left( \frac{r}{r_*} \right)^{3/2}\;.
\end{equation}
We thus see that the energy is screened with respect to the distance to the massive object. There is no factor involving the distance between the two bodies $d$. We will now evaluate precisely the scalar energy in the case of a circular orbit.

\subsection{The case of circular orbits}
In this subsection we will evaluate the two-body scalar energy for circular orbits.
Using the notations of Section~\ref{subsec:param}, we find, when $\vert \vec d \vert \lesssim \vert \vec r \vert$,
\be
\vec \rho_{1,2}\simeq \frac{1}{r^{1/2}r_\star ^{1/2}} \vec r + \frac{1}{r^{1/2}r_\star ^{1/2}} (\vec r_{1,2}-\vec r) - \frac{1}{2} ((\vec r_{1,2}-\vec r).\vec r) \frac{\vec r}{r_\star^{1/2} r^{5/2}}\;,
\ee
which imply that to leading order
\begin{align}
\rho_{1,2} &\simeq \frac{r^{1/2}}{r_\star^{1/2}} \\
\vert \vec \rho_1 -\vec \rho_2\vert &\simeq \frac{d}{r_\star^{1/2}r^{1/2}} \sqrt {1 - \frac{3}{4} \sin^2 \hat b \sin^2 \Omega t} \; .
\end{align}
As stated just above, the leading term in the two-body energy \eqref{eq:energy} is the last one,
\begin{equation}
E \simeq - 4 G \beta_\mathrm{eff}^2 \frac{m_1 m_2}{d \sqrt{1 - \frac{3}{4} \sin^2 \hat b \sin^2 \Omega t }} \left( \frac{r}{r_*} \right)^{3/2} \; .
\end{equation}

By averaging over time, we see that the effect of the scalar energy, when added to the gravitational energy $E_\mathrm{gr} = - G m_1 m_2/d$, is just a renormalization of Newton's constant $G \rightarrow G_\mathrm{eff}$, where the effective gravitational coupling constant takes the form
\begin{equation}
G_\mathrm{eff} = G \left(1 + \alpha \beta_\mathrm{eff}^2 \left( \frac{r}{r_*} \right)^{3/2}  \right) \; ,
\end{equation}
with $\alpha$ denoting a numerical quantity given by
\begin{equation}
\alpha = \frac{4}{\pi} \left[ K \left( \frac{3 \sin^2 \hat b}{4} \right) + \frac{2}{4 - 3 \sin^2 \hat b} K \left( \frac{3 \sin^2 \hat b}{3 \sin^2 \hat b - 4} \right) \right] \; ,
\end{equation}
and $K$ is the complete elliptic integral of the first kind,
\begin{equation}
K(m) = \int_0^\frac{\pi}{2} \frac{d u}{\sqrt{1 - m \sin^2 u}} \; .
\end{equation}
This result corroborates  the expectation that the two-body scalar energy is a $\beta_\mathrm{eff}^2$ correction screened by the Vainshtein factor $(r/r_*)^{3/2}$.

\section{Dissipated power} \label{sec:diss_power}
In this section we  compute the dissipated power in scalar radiation due to the presence of the cubic Galileon. The power emitted in the tensor sector will follow the usual quadrupole formula and hence we will focus on the scalar sector.

\subsection{Energy-momentum tensor}
The total energy-momentum tensor splits into gravitational and scalar contributions,
\begin{equation}
T_{\mu \nu} = T^\varphi_{\mu \nu} + T^g_{\mu \nu} \; ,
\end{equation}
where $T^g_{\mu \nu}$ is the usual Landau-Lifschitz pseudo-tensor, and $T^\varphi_{\mu \nu} = - 2 / \sqrt{-g} \delta S_\varphi/\delta g^{\mu \nu}$, where $S_\varphi$ is the scalar part of the action. Far from matter sources the total energy-momentum tensor is conserved, which allows to find the power lost into radiation by integrating it over a distant sphere of radius $\mathcal{R}$ centered on the system,
\begin{equation}
P = - \int d^2 S T_{0i}n^i = - \mathcal{R}^2 \int d^2 \Omega T_{0r} \; ,
\end{equation}
where $n^i$ is the outward pointing vector of the sphere. The Landau-Lifschitz pseudo-tensor will give rise to the usual quadrupole formula at lowest order in the post-Newtonian expansion, so there remains only to find the scalar dissipated power. The scalar energy-momentum tensor calculated from the action \eqref{eq:base_action} reads
\begin{align}
\begin{split} \label{eq:EMT}
T^\varphi_{\mu \nu} &= \partial_\mu \varphi \partial_\nu \varphi - \frac{1}{2} g_{\mu \nu} (\partial \varphi)^2 + \frac{1}{\Lambda^3} \left( \partial_\mu \varphi \partial_\nu \varphi \square \varphi + \frac{1}{2} g_{\mu \nu} \partial_\alpha \big( (\partial \varphi)^2 \big ) \right. \\
&- \left. \frac{1}{2} \big [ \partial_\mu \big( (\partial \varphi)^2 \big) \partial_\nu \varphi + \mathrm{sym} \big ]  \right) \; .
\end{split}
\end{align}
Splitting the field $\varphi = \varphi_0 + \psi$ as in Eq. \eqref{eq:action_expanded}, one can collect the terms quadratic in $\psi$ in the energy-momentum tensor. The linear terms average to zero in time in the dissipated power. As emphasised in Section~\ref{sec:setup_chap8}, the dominant terms will be the quadratic ones coming from the Galileon term. By neglecting angular and time total derivatives, which, once again, will average to zero in the dissipated power, one finds the $0r$ part of the scalar energy-momentum tensor
\begin{equation}
T^\varphi_{0r} = \frac{4  \varphi_0'}{\Lambda^3 \mathcal{R}} \partial_t \psi \partial_r \psi.
\end{equation}
For a wave travelling far from the massive objects, one has $\partial_r \psi = - \partial_t \psi / c_r$ where $c_r = \sqrt{3}/2$ is the radial propagation speed. This gives
\begin{equation} \label{eq:power_chap8}
P = \frac{8}{\sqrt{3}} \mathcal{R}^{1/2} r_*^{3/2} \int d^2 \Omega (\partial_t \psi)^2\;.
\end{equation}

\subsection{Dissipated power}

%Let us now find the field radiated at infinity. We will assume a slow motion of the small bodies $v \ll 1$ and expand all quantities in powers of the velocity. As we deal with scalar fields, there will generally be monopole and dipole radiation on top of the quadrupole one. Generically, each $n$-pole is suppressed by $v^{2n}$ in the velocity expansion with respect to the monopole.
%
%Before dealing with the calculations, let us review briefly the generic results obtained in the simpler setup of scalar-tensor theories {\bf CITATION}. In these theories, the lowest-order monopole is simply proportional to the total mass of the system and so does not radiate since it is conserved. On the other hand, if the scalar charges of the two objects are different, then there will be a dipole radiation enhanced by $1/v^2$ with respect to the quadrupole, and suppressed by the difference of scalar charges of the two objects. If the two objects share the same scalar charge, then by conservation of momentum there is no dipole radiation at lowest order.
%
%Let us now return to the Galileon case and assume that the two objects share different scalar charges, $\beta_1 \neq \beta_2$. The massive central object is assumed to have another scalar charge $\beta_0$. We will see that the lowest order contribution to the monopole is proportional to the difference of scalar charges of the two objects, $\beta_1 - \beta_2$.
%
%{\bf TODO : I IMPLICITELY ASSUME HERE THAT THE MOTION OF THE BINARY SYSTEM AROUND THE CENTRAL BLACK HOLE IS SLOW...}


Let us now find the power radiated at infinity, which reduces to finding $\psi(\vec x,t)$ at large distance from the source. In order to find the lowest-order power emitted we will assume that the two objects follow non-relativistic trajectories. The trace of their energy-momentum tensor is given by
\begin{equation}
T = - m_1 \delta^3(\vec{x} - \vec{x}_1)- m_2 \delta^3(\vec{x} - \vec{x}_2)\;.
\end{equation}
If one wanted to find higher-order corrections to the dissipated power, one would need to add relativistic corrections to this equation, but this is unnecessary for the lowest-order power as we argue below. By using eqs. \eqref{eq:field_green_fct} and \eqref{eq:green_fourier}, one finds
\begin{align}
\begin{split} \label{eq:field}
\psi(\vec x, t) &= \frac{\beta_\mathrm{eff}}{\mpl} \int dt' \frac{d\omega}{2\pi} e^{-i \omega(t-t')} \sum_{l,m} Y_l^m(\theta, \phi) \\
& \times \left[ m_1 R_{l\omega}(\mathcal{R}, \vert \vec r + \vec d_1(t') \vert) \bar Y_l^m (\theta_1(t'), \phi_1(t')) + (1 \leftrightarrow 2) \right] \; ,
\end{split}
\end{align}
where $\mathcal{R}, \theta, \phi$ are the coordinates of the distant sphere of integration (at large distance, we can set the centre-of-mass of the binary system and the position of the large mass $m_0$ to the same point), and $\theta_1(t), \phi_1(t)$ are the polar coordinates of the object 1 when taking the central mass to be the origin of the coordinates.

Equation \eqref{eq:field} represents the field in the frame corotating with the system. It is easy to find the field in the static frame attached to the central BH: one just has to replace $\phi_i(t') \rightarrow \phi_i(t') + \Omega_0 t'$ (where $\Omega_0$ is the angular speed of rotation of the barycentre of the system around the massive black hole)  in the spherical harmonics, which adds a time dependent factor $e^{-i m \Omega_0 t'}$ to the total expression.

We can then use that, for a $T$-periodic function $f$, the Fourier series becomes
\begin{equation}
\int dt' e^{i \omega t'} f(t') = 2 \pi \sum_{n \in \mathbb{Z}} c_n(f) \delta(\omega - n \Omega), \quad c_n(f) = \frac{1}{T} \int_0^T dt' f(t') e^{i n \Omega t'} \; .
\end{equation}
We find that
\begin{align}
\begin{split}
\psi(\vec x, t) &= \beta_\mathrm{eff} \frac{ (m_1+m_2)}{\mpl} \sum_{n \in \mathbb{Z}} e^{-i (n \Omega + m \Omega_0) t} \sum_{l,m} Y_l^m(\theta, \phi) (c_{n}(f_1^{lm}) + (1 \leftrightarrow 2)) \\
f_i^{lm}(t) &= X_i R_{l\omega}(\mathcal{R}, \vert \vec r + \vec d_i(t') \vert) \bar Y_l^m (\theta_i(t'), \phi_i(t')) \; ,
\end{split}
\end{align}
where $X_1 = X = m_1/(m_1+m_2)$, $X_2=1-X$ and $\omega = n \Omega + m \Omega_0$.
Finally, using eq. \eqref{eq:power_chap8} and integrating over a sphere, the total power is
\begin{equation} \label{eq:power_cn}
P = \frac{8}{\sqrt{3}} \beta_\mathrm{eff}^2 \mathcal{R}^{1/2} r_*^{3/2} \frac{(m_1+m_2)^2}{\mpl^2} \sum_{n \in \mathbb{Z}} \sum_{l,m} (m \Omega_0 + n \Omega)^2  \vert c_n(f_1^{lm}) + c_n(f_2^{lm}) \vert^2\;.
\end{equation}
At this point we can check the convergence of the different sums. The expansion in $l$ involves the mode fonction $R_{l\omega}(\mathcal{R}, x_i)$ (denoting $ x_i = \vert \vec x_i \vert = \vert \vec r + \vec d_i \vert$). More precisely, it involves a Bessel function evaluated in $x_i \Omega$. In realistic situations, one has $r \Omega \lesssim 10^{-1}$ so that we can evaluate the Bessel function for small arguments and each order in $l$ is  suppressed by $(r \Omega)^{(l+1)/2}$ (apart from the monopole whose scaling is different as we show below).
Terms in the n-expansion  arise by expanding the distance $x_i \simeq r + d_i \sin\hat b \sin(\Omega t) + \dots$ in powers of $d/r$ leading to  Fourier coefficients from the corresponding power of $\sin(\Omega t)$. Thus, the expansion in $n$ corresponds to an expansion in $d/r$.

\subsection{Monopole}

The monopole ($l=m=0$) term is simple as the spherical harmonics are given by $Y_0^0 = 1/\sqrt{4\pi}$. From eq. \eqref{eq:mode_functions}, the mode function $R_{0\omega}$ for large value of $\mathcal{R}$ is given by
\begin{align}
\begin{split}
R_{0\omega}(\mathcal{R}, x_i) &= R^2(x_i)\left( R^1(\mathcal{R}) + \frac{1}{1+i} R^2(\mathcal{R}) \right) \\
&= \frac{\sqrt{2 \pi}(1-i)}{8 \cdot 3^{1/4} r_*^{3/2} \omega^{1/2}} \left( \frac{ x_i}{\mathcal{R}} \right)^{1/4} e^{i \sqrt{3} \omega \mathcal{R}/2 - i 3\pi/8} J_{-1/4}\left( \frac{\sqrt{3}}{2} x_i \omega \right) \; ,
\end{split}
\end{align}
where we have used the behaviour \eqref{eq:asymptotic_bessel} at infinity.
One can then Taylor expand the Bessel function as $x_1 \simeq r + d_1 \sin\hat b \sin(\Omega t) + \dots$ and  $d \lesssim r$. As the scalar field is real  only the even powers of  $(d/r)^{2k}$ appear in the sum of the Fourier coefficients $c_n(f_1) + c_n(f_2)$. They arise as $d$ accompanies  $ \sin(\Omega t)$ in the expansion and  terms of order $d^{2k}$ will only give contributions to harmonics of order  $n \leq 2k$.

Since the constant $n=0$ term does not give any power in monopole (see eq. \eqref{eq:power_cn}), the lowest-order contribution is given by $n=2$ (so $\omega = 2 \Omega$) with at second order in $d/r$
\begin{align}
\begin{split} \label{eq:cn_monopole}
c_2(f_1^{00}) + c_2(f_2^{00}) &=  X(1-X) J_{7/4}\left( \sqrt{3} r \Omega \right) \sin^2(\hat b) \\
&\times (1-i)e^{ i \sqrt{3} \Omega \mathcal{R}/2 - i 3\pi/8} \frac{3^{3/4}}{2^7} \frac{ r^{1/4} (d \Omega)^2}{\mathcal{R}^{1/4} \Omega^{1/2} r_*^{3/2}} \; .
\end{split}
\end{align}
An important observation is that this second-order expansion depends on $(d\Omega)^2$ and not on $(d/r)^2$. Since in realistic physical situations $d/r \sim 1/50$ while $d \Omega \sim 10^{-3}$, this makes the monopole much more suppressed than the other modes. Another important point to notice is that relativistic corrections to the energy-momentum tensor as well as couplings between gravity and the field $\psi$ would correct this expression with terms scaling precisely as $(d \Omega)^2$. Thus, since a precise evaluation of the monopole would require these terms as well. We move on to the calculation of the dipole.

\subsection{Dipole}

The dipole term is defined by $l=1$, $m =0, \pm 1$. The mode function $R_{1 \omega}$ is given by
\begin{align}
\begin{split} \label{eq:mode_fonction_dipole}
R_{1\omega}(\mathcal{R}, x_i) &= - R^1(x_i)\left( R^2(\mathcal{R}) + (1-i) R^1(\mathcal{R}) \right) \\
&= - \frac{\sqrt{2 \pi}}{4 \cdot 3^{1/4} r_*^{3/2} \omega^{1/2}} \left( \frac{ x_i}{\mathcal{R}} \right)^{1/4} e^{i \sqrt{3} \omega \mathcal{R}/2 - i 5\pi/8} J_{3/4}\left( \frac{\sqrt{3}}{2} x_i \omega \right) \; ,
\end{split}
\end{align}

 We split up the computation between $n=0$, which represents the dipolar emission of the centre-of-mass due to its motion around the central mass and $n=2$ which contains also dipolar emission from the motion of the small masses themselves around their centre-of-mass.

\subsubsection{$n=0$ term} \label{sec:dip_n0}

The $n=0$ term corresponds to replacing $x_i \rightarrow r$ at lowest order in the $d/r$ expansion. Only the $m = \pm 1$ modes radiate (see eq. \eqref{eq:power_cn}). The relevant spherical harmonics are given by
\begin{equation}
Y_1^1(\theta, \phi) = - \bar Y_1^{-1}(\theta, \phi) = - \sqrt{\frac{3}{8 \pi}} \sin \theta e^{i \phi} \; .
\end{equation}
Moreover, with the replacement $x_i \rightarrow r$, i.e positions are evaluated at the barycentre of the system, one has $\theta_i = \phi_i = 0$. Using the expression for the mode function \eqref{eq:mode_fonction_dipole} it is easy to find
\begin{equation} \label{eq:dipole_n0term}
P_{n=0} = \frac{\beta_\mathrm{eff}^2}{4} J_{3/4}^2\left( \frac{\sqrt{3}}{2} r \Omega_0 \right) \frac{(m_1+m_2)^2}{\mpl^2} \left( \frac{r}{r_*} \right)^{1/2} \frac{\Omega_0}{r_*}
\end{equation}

Let us evaluate the order-of-magnitude of this expression for $r \Omega_0 \lesssim 1$. We find
\begin{equation}
P_{n=0} \sim \frac{\beta_\mathrm{eff}^2}{G} \frac{1}{(\Omega_0 r_*)^{3/2}} \left( \frac{m_i}{m_0} \right)^2 v^8
\end{equation}
where we have used the variable $v$ defined as $v=(G m_0 \Omega_0)^{1/3}$, which scales as a velocity in the post-Newtonian expansion and is related to the radius using Kepler's third law
\begin{align}
r = \left( \frac{G m_0}{\Omega_0^2} \right)^{1/3}.
 \equiv G m_0 v^{-2}
\end{align}
Comparing to the GR quadrupole power loss of a point-particle in circular orbit, $P_\mathrm{GR} \sim (m_i/m_0)^2 v^{10} / G$, we see that the dipole emission is enhanced by two powers of the velocity (as expected), but is suppressed by the Vainshtein factor $1/(\Omega_0 r_*)^{3/2}$, in line with the findings of Refs.~\cite{deRham:2012fg,dar_scalar_2018,deRham:2012fw}. This factor is extremely small as long as the Vainshtein radius is much larger than the size of the system, more precisely the wavelength of the emitted radiation. This implies that the  Vainshtein screening is  quite efficient for the global motion of the barycentre around the central mass, even if the dipolar power is generically enhanced by two powers of the velocity.

\subsubsection{$n=2$ term}

As explained above, only the even $n$ can contribute to the power. Let us first concentrate on the $m=0$ term, which is the most interesting because it does not involve the rotation $\Omega_0$ around the massive black hole and so represents a power loss for the binary system itself. The expression for the $l=1,m=0$ spherical harmonic is
\begin{equation}
Y_1^0(\theta, \phi) = \sqrt{\frac{3}{4 \pi}} \cos(\theta) \; .
\end{equation}

Let us choose $\theta$ and $\phi$ such that the barycentre of the system lies in the $\theta=\pi/2$ plane and such that this plane is perpendicular to the $x$ axis (of unit vector $\hat x$). Then trigonometry gives
\begin{equation}
\cos \theta_i = \frac{\vec d_i \cdot \hat x}{\sqrt{r^2 + (d_i \cdot \hat x)^2}} \; ,
\end{equation}
where $\theta_i$ is the $\theta$ angle of the object $i=1,2$. With this in hand, one can compute the Fourier coefficient
\begin{align}
\begin{split}
c_2(f_1^{10}) + c_2(f_2^{10}) &= \left(  X(1-X) J_{3/4}\left( \sqrt{3} r \Omega \right) \sin(\hat b) + \mathcal{O}(r \Omega) \right) \\
&\times i e^{ i \sqrt{3} \Omega \mathcal{R} - i 5\pi/8} \frac{3^{1/4}}{32 r_*^{3/2} \Omega^{1/2}} \left( \frac{r}{\mathcal{R}} \right)^{1/4} \frac{ d^2}{r^2} \; ,
\end{split}
\end{align}
where we have kept the leading term in $r \Omega$, and the $X(1-X)$ prefactor comes from replacing $d_i \rightarrow X_i d$. We thus confirm our previous claim: comparing to eq. \eqref{eq:cn_monopole}, we see that this term involves the small parameter $d/r$ instead of the much smaller one $d \Omega$. Thus, the dipole will dominate the dissipated power.

Replacing in the expression of the Fourier coefficients for the power (by symmetry, for $m=0$ the positive and negative $n$ give  the same contribution to the power) we find
\begin{equation}
P_{n=2, m=0} = \frac{\beta_\mathrm{eff}^2}{16} \frac{(m_1+m_2)^2}{\mpl^2} \frac{\Omega d^4}{r^{7/2} r_*^{3/2}} X^2(1-X)^2  J_{3/4}^2\left( \sqrt{3} r \Omega \right) \sin^2(\hat b)
\end{equation}

Introducing as for the $n=0$ term the variable $u=(G (m_1+m_2) \Omega)^{1/3}$, related to $d$ via
\begin{align}
d = \left( \frac{G (m_1+m_2)}{\Omega^2} \right)^{1/3}
 \equiv G (m_1+m_2) u^{-2}
\end{align}
we can rewrite the power as
\begin{equation} \label{eq:new_scalar_power}
P_{n=2, m=0} = \frac{\pi \beta_\mathrm{eff}^2}{2G} \left( \frac{r}{r_*} \right)^{3/2} \left( \frac{G(m_1+m_2)}{r} \right)^5 u^{-5} X^2(1-X)^2  J_{3/4}^2\left( \sqrt{3} r \Omega \right) \sin^2(\hat b) \; .
\end{equation}

The negative power in front of $u$ could seem worrisome as it diverges for small velocities, but recall that we are expanding in $d/r$ so $d$ cannot be taken to infinity without invalidating our expansion. Let us compare this expression with the GR quadrupole of a binary system in isolation $P_\mathrm{GR} \sim u^{10}/G$. Expanding the Bessel function for small arguments, we find
\begin{equation}
\frac{P_{n=2, m=0}}{P_\mathrm{GR}} \sim \beta_\mathrm{eff}^2 \left( \frac{r}{r_*} \right)^{3/2} \left( \frac{G(m_1+m_2)}{r} \right)^{7/2} u^{-21/2}
\end{equation}

With the orders-of-magnitude given in the introduction, one can evaluate this ratio to be
\begin{equation}
\frac{P_{n=2, m=0}}{P_\mathrm{GR}} \sim 10^{3} \beta_\mathrm{eff}^2 \left( \frac{r}{r_*} \right)^{3/2}
\end{equation}

Just as we proved in Section~\ref{sec:dip_n0} that the Vainshtein screening is efficient for the motion of the barycentre of the system around the central mass, we see  that it is also  efficient for the motion of the binary system itself apart from a small enhancement factor of order $10^3$ ( recall that $(r/r_*)^{3/2} \sim 10^{-16}$ for a cosmological Galileon). In the next Section, we will compute the modification to the phase induced by this new power loss by assuming it is a small correction to the GR quadrupole. This is valid as long as $\beta_{\rm eff} \lesssim 10^7$ which we assume in the following.

%In particular for large enough $\beta_\mathrm{eff}\gtrsim 10^3$, the power emitted in the scalar radiation modes can be larger than the quadrupole radiation from GR. We will investigate this regime further below.

Finally, one can also compute the term in the dissipated power coming from the harmonics $m=\pm 1$ with the same strategy, giving a result
\begin{align}
 \begin{split}
P_{n=2, m=\pm 1} &= \frac{9 \beta_\mathrm{eff}^2}{512} \frac{(m_1+m_2)^2}{\mpl^2} \frac{d^4}{r^{7/2} r_*^{3/2}} X^2(1-X)^2 \sin^4(\hat b) \\
& \times \left((2 \Omega + \Omega_0)  J_{3/4}^2\left(\frac{ \sqrt{3}}{2} r (2 \Omega + \Omega_0) \right) + \vert 2 \Omega - \Omega_0 \vert  J_{3/4}^2\left(\frac{ \sqrt{3}}{2} r \vert 2 \Omega - \Omega_0 \vert \right) \right) \; .
\end{split}
\end{align}
This term involves a mixing between the two-body trajectory (parameterised by $\Omega$) and the revolution around the central black hole (parameterised by $\Omega_0$). With the conditions $\Omega_0 \gtrsim \Omega$ and $d/r \lesssim 1$, this is a subleading correction compared to the $n=0$ term \eqref{eq:dipole_n0term}.

\section{Inspirals and scalar correction to the phase} \label{sec:inspiral}
%and place ourselves in the situation where $r$ can be taken as constant (in other words, the binary inspiral induced by the scalar power is sufficiently quick so that we can ignore the motion around the central black hole)

Here we compute the scalar correction to the GW phase recorded in a detector such as LISA. Within our simple approximation scheme, there are two kind of GW signals: the one caused by the motion of the centre-of-mass around the supermassive BH (at a frequency $\Omega_0$), as well as the motion of the binary around its own centre-of-mass (at a frequency $\Omega$). We make the assumption that each of these two motions can be treated separately - the so-called "Hill's approximation" - and we compute the relevant scalar phase in the two following subsections.

\subsection{Extreme mass-ratio inspiral} \label{sec:EMRI}

In this Section, we will compute the modification to the GW phase (due to scalar wave emission) of the inspiral of the binary as a whole around the massive BH. Alternatively, our equations will be valid for any extreme-mass ratio inspiral of a light object around a massive BH provided once replaces the total mass $m_1+m_2$ by the mass of the small object. This will allow us to derive a lower bound on the effective coupling $\beta_\mathrm{eff}$ in order to be able to detect a Galileon correction to the GW phase.

Since the scalar power loss is enhanced by the fact that it is a dipole, we will compute the phase assuming that it induces the leading deviation from GR (the scalar correction to the energy is 'usually' Vainshtein suppressed, i.e. it does not involve a dipolar enhancement, so we will neglect it).
The relevant dipolar power correction is given by equation \eqref{eq:dipole_n0term}. We still assume that the GR quadrupole dominates the power loss.

Using Kepler's third law, the Newtonian energy of the system is
\be
E = - \frac{(m_1+m_2)^2 v^2}{2 m_0} \; ,
\ee
where we recall that $v = (Gm_0 \Omega_0)^{1/3}$. The time evolution of the binary system is given by the balance equation
\begin{equation} \label{eq:balance}
\frac{dE}{dt}= -P_{GR}- P_\phi \; ,
\end{equation}
where $P_\phi$ is the scalar power loss for the $n=0$ dipole term in Eq. \eqref{eq:dipole_n0term} (with the Bessel function expanded for small arguments) and $P_\mathrm{GR}$ is the GR quadrupolar power loss given by
\begin{equation}
P_\mathrm{GR} = \frac{32}{5G} \left( \frac{m_1+m_2}{m_0} \right)^2 v^{10}
\end{equation}
Let us introduce the dimensionless constant $C_1$ by $P_\phi = C_1 P_\mathrm{GR} v^{-13/2}$, i.e.
\begin{equation}
C_1 = \frac{5 \times 3^{3/2} \pi \beta_\mathrm{eff}^2}{128 \Gamma(7/4)^2} \left( \frac{Gm_0}{r_*} \right)^{3/2} \; .
\end{equation}
The balance equation \eqref{eq:balance} then takes the form
\begin{equation}
\frac{dv}{dt} = \frac{32 (m_1+m_2)}{G m_0^2} v^9 \left( 1 + C_1 v^{-13/2} \right) \; .
\end{equation}
The number of observable GW cycles of the binary system in the detector is $2 \Phi(t)$ where
\begin{equation}
\Phi(t)= \int_{t_\mathrm{in}}^t \Omega_0 dt= \frac{1}{Gm_0} \int_{v_\mathrm{in}}^v dv v^3 \left(\frac{dt}{dv}\right) \; ,
\end{equation}
where $t_\mathrm{in}$ is the initial time at which the signal enters in the GW detector, and $v_\mathrm{in}=v(t_\mathrm{in})$.

Assuming a final velocity $v_\mathrm{out} \sim 1$ when the binary system plunges into the central BH, the total accumulated phase during the inspiral is $\Phi = \Phi_\mathrm{GR} + \Delta \Phi$ where $\Phi_\mathrm{GR}$ is the usual GR phase,
\begin{equation}
\Phi_\mathrm{GR} = \frac{1}{32} \frac{m_0}{m_1+m_2} v_\mathrm{in}^{-5} \sim 10^7 \; ,
\end{equation}
and $\Delta \Phi$ is the correction due to the scalar field,
\begin{equation}
\Delta \Phi = \frac{10}{736}  \frac{m_0}{m_1+m_2} C_1 v_\mathrm{in}^{-23/2} \; .
\end{equation}
With the order-of-magnitudes given in the introduction and expanding in all the relevant parameters, we find
\begin{equation} \label{eq:delta_phi_EMRI}
\Delta \Phi \simeq 10^{-6} \beta_\mathrm{eff}^{3/2} \left( \frac{\Lambda}{10^{-12} \mathrm{eV}} \right)^{3/2} \; \left( \frac{m_1+m_2}{60 M_\odot} \right)^{-1} \; \left( \frac{m_0}{10^6 M_\odot} \right)^{-11/6} \; \left( \frac{\Omega_\mathrm{in}}{10^{-3} \mathrm{Hz}} \right)^{-23/6} \; ,
\end{equation}
where $\Omega_\mathrm{in}$ is the minimal frequency at which the GW signal is observed in the detector. Let us emphasize again that this formula is valid for any extreme-mass ratio inspiral of a small object of total mass $m_1+m_2$ onto a supermassive BH.

The precision achieved on the phase of GW observatories is at the level of $\Delta \Phi \sim 0.1$~\cite{Babak_2017}, so that an effective scalar charge $\beta_\mathrm{eff} \gtrsim 10^4$ would induce observable modifications to the GW phase. Note that $\Delta \Phi$ is quite sensitive to the minimal frequency $\Omega_\mathrm{in}$ at which the signal is detected in the interferometer, so that a lower $\Omega_\mathrm{in}$ would greatly increase the detectability of such an event. Likewise, a value of $\Lambda \sim 10^{-8}$ eV would allow for a detection with $\beta_\mathrm{eff} \sim 1$.



\subsection{Binary inspiral}

We now concentrate on the GW signal originating from the motion of the binary system around its centre-of-mass, entering a detector at frequency $\Omega$.
We make the assumption that the new formula we found for the enhanced scalar dissipated power in Eq. \eqref{eq:new_scalar_power} dominates the scalar loss of energy of the binary system, while the conservative energy is still dominated by GR, since the scalar energy is Vainshtein suppressed from Eq. \eqref{eq:energy}. We still assume that the GR quadrupole dominates the power loss and we will compute the modification to the phase of the GW as in the previous Section.



% This can be the case for moderately large values of the effective coupling
%$\beta_{\rm eff}$. More precisely and using Kepler's third law the energy of the binary system can be written as

The Newtonian energy of the binary system is
\be
E = - \frac{(m_1+m_2) \nu u^2}{2} \; ,
\ee
where $\nu=\frac{\mu}{m_1+m_2}$, $\mu=\frac{m_1m_2}{m_1+m_2}$ and we recall that $u = \left( G (m_1+m_2) \Omega \right)^{1/3}$. The balance equation takes the same form,
\be
\frac{dE}{dt}= -P_{GR}- P_\phi \; ,
\ee
where $P_\phi$ is the scalar power loss for the $m=0$ dipole term in Eq. \eqref{eq:new_scalar_power} and $P_\mathrm{GR}$ is the GR quadrupolar power loss given by
\begin{equation}
P_\mathrm{GR} = \frac{32}{5G} \nu^2 u^{10}
\end{equation}
Let us introduce the dimensionless 'constant' $C$ by writing $P_\phi= C \nu^2 u^{-1/2} / G$, i.e
\begin{equation}
C=\frac{3^{3/4} \pi \beta_\mathrm{eff}^2}{4 \sqrt{2} \Gamma(7/4)^2} \left( \frac{r}{r_*} \right)^{3/2} \left( \frac{G(m_1+m_2)}{r} \right)^{7/2}   \sin^2(\hat b)
\end{equation}
where once again we have expanded the Bessel function in eq. \eqref{eq:new_scalar_power} for small arguments. For the largest possible $r$ allowed by our condition \eqref{eq:condition_green} one has $C \sim 10^{-39} \beta_\mathrm{eff}^2$, but for smaller $r$, $C$ increases as $r^{-2}$.  Then the time evolution of $u$ is given by
\begin{equation} \label{eq:dudt}
\frac{d u}{d t} = \frac{\nu}{G(m_1+m_2)} \left( \frac{32}{5} u^9 + C u^{-1/2} \right)
\end{equation}
In the regime where the first term coming from the GR quadrupole dominates, we have
\begin{equation} \label{eq:ut}
u(t)= u_\mathrm{in}\left( 1-  \frac{(t-t_\mathrm{in})}{t_1} \right)^{-1/8} \; ,
\end{equation}
where
\be
t_1=\frac{5}{256} \frac{G(m_1+m_2)}{\nu u_\mathrm{in}^8}=\frac{5}{256}\frac{d_\mathrm{in}^4}{G^3 (m_1+m_2)^3 \nu} \; ,
\ee
is the time of collapse from the initial time $t_\mathrm{in}$ where $u_\mathrm{in}=u(t_\mathrm{in})$, $d_\mathrm{in}=d(t_\mathrm{in})$, which we choose to be the time at which our perturbative calculation is valid according to Eq. \eqref{eq:condition_green}.

However, the binary system will always fall into the central BH before merging itself. This is because the time of collapse into the central BH is
\begin{equation}
t_0 = \frac{5}{256} \frac{Gm_0^2}{(m_1+m_2) v_\mathrm{in}^8} \; ,
\end{equation}
as the reduced mass is $m_1+m_2$ and the mass of the central object is $m_0$, and we recall that we have introduced the variable $v=(G m_0 \Omega_0)^{1/3}$. Since at the initial time where the perturbative calculation begins to be valid one has $\Omega_0^\mathrm{in} = \Omega^\mathrm{in}$ (see the comment at the end of Section~\ref{subsec:param}), the ratio of the collapse times is
\begin{equation}
\frac{t_0}{t_1} = \left( \frac{m_1 + m_2}{m_0} \right)^{2/3} \sim 10^{-3} \; .
\end{equation}

Before being swallowed by the central BH, the binary system would still produce GW. The number of observable GW cycles of the binary system in the detector is $2 \Phi(t)$ where
\begin{equation}
\Phi(t)= \int_{t_\mathrm{in}}^t \Omega dt= \frac{1}{G(m_1+m_2)} \int_{u_\mathrm{in}}^u du u^3 \left(\frac{dt}{du}\right) \; .
\end{equation}
Let us compute first the number of cycles assuming that the power loss is purely GR. One finds
\begin{equation}
\Phi = \frac{1}{32 \nu} \left( u_\mathrm{in}^{-5} - u_\mathrm{out}^{-5} \right) \; ,
\end{equation}
where $u_\mathrm{out} = u(t_0)$ is the value of $u$ when the binary system plunges inside the massive BH. Expanding Eq. \eqref{eq:ut} for $t_0 / t_1 \ll 1$, one finds
\begin{equation}
\Phi \simeq \frac{5}{256} u_\mathrm{in}^{-5} \frac{t_0}{t_1} \sim 10^7 \; ,
\end{equation}
which shows that the signal would be observable during a fairly large amount of cycles. Let us now compute the correction to the phase due to the scalar power loss. Expanding equation \eqref{eq:dudt} for small $C$, it is
\begin{equation}
\Delta \Phi = \frac{25}{1024 \nu} \int \mathrm{d} u \; C u^{-31/2}
\end{equation}
In the integral, $C$ depends on time (so it depends on $u$) \textit{via} its dependence on $r$. We make the simplifying assumption that $r$ decreases according to the quadrupole formula, i.e.
\begin{equation}
r = r_\mathrm{in} \left( 1 - \frac{t-t_\mathrm{in}}{t_0} \right)^{1/4}
\end{equation}
We can relate $t-t_\mathrm{in}$ to $u$ using Eq. \eqref{eq:ut} expanded for $t/t_1 \ll 1$. Since $C \propto r^{-2}$, this gives
\begin{equation}
\Delta \Phi = \frac{25}{1024 \nu} C_\mathrm{in} u_\mathrm{in}^{-29/2} \int_1^{1+\frac{t_0}{8t_1}} \mathrm{d} x \; x^{-31/2} \left(1 - 8 \frac{t_1}{t_0} \left(x - 1 \right)  \right)^{-1/2} \; ,
\end{equation}
where we have used the change of variable $x = u/u_\mathrm{in}$. Expanding once again for $t_0/t_1 \ll 1$, we finally find
\begin{equation}
\Delta \Phi = \frac{25}{4096 \nu} C_\mathrm{in} u_\mathrm{in}^{-29/2} \frac{t_0}{t_1} \; .
\end{equation}
With the order-of-magnitudes given in the introduction and expanding in all the relevant parameters, we find
\begin{equation} \label{eq:delta_phi_binary}
\Delta \Phi \simeq 10^{-7} \beta_\mathrm{eff}^{3/2} \left( \frac{\Lambda}{10^{-12} \mathrm{eV}} \right)^{3/2} \; \left( \frac{m_1+m_2}{60 M_\odot} \right)^{-2/3} \; \left( \frac{m_0}{10^6 M_\odot} \right)^{-11/6} \; \left( \frac{\Omega_\mathrm{in}}{10^{-3} \mathrm{Hz}} \right)^{-7/2}
\end{equation}

This result is similar to the one that we obtained above \eqref{eq:delta_phi_EMRI}, with slightly different powers of the parameters. Again for $\beta_{\rm eff}\gtrsim 10^4$ we could expect to detect the inspiralling phase of the two BHs falling towards each other.


%On the contrary when the emitted power is mainly due to the scalar field, we have
%\be
%u(t)=u_\mathrm{in}\left(1+\frac{(t-t_\mathrm{in})}{t_{\pi}}\right)^{2/3}
%\ee
%where we have introduced
%\be
%t_\pi= \frac{2G(m_1+m_2) u_\mathrm{in}^{3/2}}{3C \nu}.
%\ee
% Scalar emission induces, in the long term, the inspiralling of the trajectory in a much slower fashion than in GR where the evolution of $u$ ends up in a singular behaviour.
%Requiring that $t_\pi \ll t_{\rm GR}$ so that effects due to the cubic Galileon are dominant, we must impose that
%\begin{equation}
%C \gg u_\mathrm{in}^{19/2} \sim 10^{-30} \; ,
%\end{equation}
%for initial conditions such that $u_\mathrm{in} \sim 10^{-3}$. Thus, for $\beta_\mathrm{eff} \gtrsim 10^{3}$ we can observe a change in the evolution of the frequency of the binary due to the presence of the cubic Galileon. Note that for these values of $\beta_\mathrm{eff}$ the Vainshtein suppression of the static energy is still quite effective so that we do not see any deviation from GR in the energy, as well as for the motion of the binary itself around the central black hole.

%TODO : abbreviation SMBH
%However, the motion of the binary system around the supermassive BH is such that it will plunge into it in a shorter time of order of magnitude
%\be
%T_{\rm GR}= \frac{5}{256} \frac{Gm_0^2}{(m_1+m_2) v_\mathrm{in}^8}
%\ee
%as the reduced mass is $m_1+m_2$ and the mass of the central object is $m_0$, and we recall that we have introduced the variable $v=(G m_0 \Omega_0)^{1/3}$. For couplings $\beta_\mathrm{eff} \lesssim 10^5$ one generically has $T_\mathrm{GR} \ll t_\mathrm{\pi}$, so that the plunge into the supermassive BH will happen before the binary system itself merges. The number of observable GW cycles of the binary system in the detector is $2 \Phi(t)$ where
%\begin{equation}
%\Phi(t)= \int_{t_\mathrm{in}}^t \Omega dt= \frac{1}{G(m_1+m_2)} \int_{u_\mathrm{in}}^u du u^3 \left(\frac{dt}{du}\right)
%\end{equation}
%Taking the derivative of $u$ to be dominated by the scalar emission in Eq.~\eqref{eq:dudt} and expanding for $T_\mathrm{GR} / t_\pi \ll 1$, one finds that after a time $T_\mathrm{GR}$ the number of cycles is approximately
%\begin{equation}
%\Phi \simeq \frac{5}{256} \left( \frac{m_0}{m_1+m_2} \right)^2 \frac{u_\mathrm{in}^3}{v_\mathrm{in}^8} \sim 10^7
%\end{equation}
%which shows that the signal would be observable during a fairly large amount of cycles.
%
%{\color{blue} I don't understand this sentence}
%On the other hand, for larger values of the coupling the scalar emission only dominates the early phase of the three-body motion. Typically the binary system will still be absorbed by the central BH before its own merging. In the final phase of this event, GR dominates and no new physics is expected.



%\be
%\beta_{\rm eff} \gg \frac{2^4}{\sqrt{35 }} \frac{\nu u_0^{15/2}}{B}
%\ee
%where we have introduced $C=\beta_{\rm eff}^2 B^2$.
%This gives typically (to be checked properly)
%\be
%\beta_{\rm eff} \gg \nu
%\ee
%for a triple system formed of a central BH orbited by a binary system of smaller BH's. Of course this is weaker than the requirement that $P_\phi\gg P_{\rm GR}$ and therefore
%we can expect that the collapse is then due to the scalar field in this large coupling regime.
%
%Finally we must compare the collapse time $t_\phi$ to $T_{\rm GR}$ which is the collapse time of the binary system viewed as a single object orbiting the central BH
%\be
%T_{\rm GR}= \frac{5}{256} \frac{Gm_0^2}{(m_1+m_2) v_0^8}
%\ee
%as the reduced mass is $m_1+m_2$ and the mass of the central object $m_0$. Requiring that $T_{\rm GR} \gg t_\phi$ leads to a condition of $\beta_{\rm eff}$
%\be
%\beta_{\rm eff} \gg \frac{2^4}{\sqrt 35} \frac{\sqrt \nu}{\sqrt u_0}(\frac{u_0}{v_0})^4 (\frac{m_1+m_2}{m_0}) \frac{1}{\sqrt{G (m_1+m_2) B^2}}
%\ee
%of order
%\be
%\beta_{\rm eff} \gg \frac{\sqrt \nu}{\sqrt u_0}(\frac{m_1+m_2}{m_0})^3 (\frac{r}{d})^2 (\frac{r}{G(m_1+m_2)})^{5/2} (\frac{r_\star}{r})^3/4
%\ee
%which implies that $\beta_{\rm eff} \gg 10^8$. Unless $\beta_{\rm eff}$ is very large (we need a discussion somewhere on the values of $\beta_{\rm eff}$ which we can expect, for instance $q$ could be induced by galactic effects so much larger than $H_0$ and therefore we could have it large?), the binary system will collapse towards the central BH before the end of the collapse unto itself. This implies that a short number of cycles in the gravitational wave signal due to the scalar field could be observed.
%The phase of the gravitational wave is $2\Phi(t)$ where
%\be
%\Phi(t)= \int_{t_0}^t \Omega dt= \frac{1}{G(m_1+m_2)} \int_{u_0}^u du u^3 (\frac{dt}{du})
%\ee
%which leads to
%\be
%\Phi(t)= \frac{\nu}{G_N(m_1+m_2) C} (u_0^{-2} - u^{-2}).
%\ee
%In Figure 2, we have represented the evolution of $u(t)$ due to both the GR quadrupole and the scalar dipole for different values of $\beta_{\rm eff}$. In Figure 3, we have shown the time evolution of $v(t)$ due to the collapse of the binary system towards the central BH and the corresponding time evolution of the phase $\Phi (t)$.

% The Fourier coefficient involves only the $n=1$ harmonic at this order of the expansion (ignoring the constant $n=0$ term which does not radiate) and one readily finds
%\begin{align}
%\begin{split}
%c_1(f_1^{00}) + c_1(f_2^{00}) &=  X(1-X)(\beta_2-\beta_1) J_{3/4}\left( \frac{\sqrt{3}}{2} r_0 \Omega \right) \sin(\beta) \\
%&\times i(1-i)e^{i \sqrt{3} \Omega \mathcal{R}/2 - i 3\pi/8} \frac{3^{1/4} \sqrt{2}}{2^7 \sqrt{\pi}} \frac{r r_0^{1/4} \Omega^{1/2}}{\mathcal{R}^{1/4} r_*^{3/2}} \; .
%\end{split}
%\end{align}



%  Let us denote by $\mathcal{A}$ the first line of this equation, depending on the distance to the massive black hole through the Bessel function. We can use the fact that, for a circular orbit,
%\begin{align}
%\begin{split}
%d &= \left( \frac{m_1+m_2}{8\pi \mpl^2 \Omega^2} \right)^{1/3} \\
%& \equiv \frac{m_1+m_2}{8\pi \mpl^2} u^{-2}
%\end{split}
%\end{align}
%where the variable $u = (G(m_1+m_2) \Omega)^{1/3}$ scales as $v$ in the post-Newtonian expansion. The dissipated power is finally
%\begin{equation}
%P_\mathrm{mono} = \frac{3 \pi}{256} \beta_\mathrm{eff}^2 \mathcal{A}^2 \frac{m_1+m_2}{r_*} \left( \frac{r_0}{r_*} \right)^{1/2} u^7
%\end{equation}



%The order-of-magnitude of the GR quadrupolar power is $M_P^2 u^{10}$. The ratio between the scalar power and the GR one is consequently, as an order-of-magnitude,
%\begin{equation}
%\frac{P}{P_\mathrm{GR}} \sim \mathcal{A}^2 \left( \frac{r_0}{r_*} \right)^{1/2} \frac{1}{\Omega r_* u^2}
%\end{equation}

%This is quite interesting ! Indeed, the usual Vainshtein energy is suppressed by $\left( \frac{r}{r_*} \right)^{3/2}$. So this one is much less suppressed !

%Of course to calculate the effect of this force we must plug in some trajectory. Since it is already quite complicated at the Newtonian level (3-body problem) we still have some work...




%Let's now find the Green function. Following~\cite{Andrews_2013}, we introduce the change of variable
%\begin{align}
%\begin{split}
%\vec{\rho} &= \sqrt{\frac{r}{r_*}} \hat{r} \\
%g(\vec{\rho}, t; \vec{\rho}', t') &= \frac{G(\vec{r}, t; \vec{r}', t')}{\rho \rho'}
%\end{split}
%\end{align}
%where $\hat{r} = \vec{r} / r$. Then it is easy to find that $g$ obeys the usual 3-dimensional Laplace problem in the variable $\rho$, i.e
%\begin{equation}
%\left[ - 3 \rho^2 \partial_t^2 + \frac{1}{\rho^2} \partial_\rho \left(\rho^2 \partial_\rho \right) + \frac{1}{\rho^2} \nabla_\Omega^2 \right] g(\vec{\rho}, t; \vec{\rho}', t') = \frac{1}{2r_*} \delta^3(\vec{\rho} - \vec{\rho}') \delta(t-t')
%\end{equation}
%where we have used
%\begin{equation}
%\delta^3(\vec r - \vec r') = \frac{1}{2 r_*^3 \rho^3} \delta^3(\vec \rho - \vec \rho')
%\end{equation}
%from which we immediately deduce that in the static case where we ignore time derivatives
%\begin{equation}
%g(\vec{\rho}, \vec{\rho}') = - \frac{1}{8\pi r_* \vert \vec{\rho} - \vec{\rho}' \vert } + \text{homogeneous solution}
%\end{equation}
%In order to find the homogeneous solution, we will use the following trick. Consider the field produced by a variation $m \rightarrow m + \delta m$ of the central mass. From eq.~\eqref{eq:spherically_sym_field} (with a field vanishing at the origin), it is
%\begin{equation}
%\delta \phi_0(r) = \frac{\beta \delta m}{8\pi \mpl r_*} \left( \frac{r}{r_*} \right)^{1/2}
%\end{equation}
%
%On the other hand, from eq.~\eqref{eq:field_green_fct}, we have
%\begin{align}
%\begin{split}
%\delta \phi_0(\vec x) &= - \frac{\beta}{\mpl} \int d^3x' G(\vec x, \vec x') T(\vec x') \\
%&= \frac{\beta \delta m}{\mpl} G(\vec x, \vec 0)
%\end{split}
%\end{align}
%
%By equating these two equations, we find the homogeneous solution. Finally, using the symmetry of the Green function by permutation of its arguments, we find that in the static case

\section{Conclusions}
\label{SecCon}

Let us recap here the main results of this Chapter. Using the Green's function of a cubic Galileon,
we have computed the scalar corrections to the conservative and dissipative dynamics of a triple system composed of a supermassive BH and two solar-size BH.

We  found that the two-body scalar energy of the binary system is suppressed by the Vainshtein factor corresponding to the distance to the supermassive BH. In the case of circular orbits, we showed that the effect of the scalar energy translates into a renormalisation of  Newton's constant. As expected, the two-body scalar energy gives a correction proportional to the effective matter coupling of the Galileon $\beta_\mathrm{eff}^2$ and is screened by the Vainshtein factor $(r/r_*)^{3/2}$ due to the central BH, where $r$ is the distance of the binary system to the central BH. 

Then we computed the dissipated power in the presence of the cubic Galileon. Due to the absence of non-minimal couplings to matter, the tensor radiation of GW waves follows the standard quadrupole formula. Crucial new effects appear  in the scalar radiation.  We computed both the dipolar emission of the centre-of-mass due to its motion around the central BH and the dipolar emission from the motion of the small masses themselves around their common  centre-of-mass. In the former, the dipole power is enhanced compared to the GR case by two powers of the velocity. Unfortunately it is still suppressed by the Vainshtein factor $1/(\Omega_0 r_*)^{3/2}$ implying that the overall scalar emission is suppressed. In the latter, we  found a velocity enhancement due to the dipolar power leading to a small reduction of the Vainshtein efficiency.


Finally, we have derived the Galileon corrections to the phase of gravitational waves emitted from the system. Since the number of cycles can be very large, the relative precision of GW observatories could be excellent allowing for detection of  tiny modifications from GR. In this respect, we have found that for large enough conformal couplings a modification to the GW phase due to the Galileon can be induced. Our results can alternatively be seen as constraints on the strong coupling scale $\Lambda$ present in all Galileon interactions.

 Of course, the configuration studied in this Chapter is very special. For BHs of masses around 30 $M_\odot$ and for frequency in the LISA band, this requires that the two BHs in the binary system should be closer than 0.01 AU and that they should be less than 0.5 AU away from the central BH; furthermore, a more realistic treatment would necessitate to take into account the higher order post-Newtonian corrections, the eccentricity of the orbit, the spins of the BH, and the accretion disk of the supermassive BH~\cite{McKernan:2019beu}. Part of our results are also valid for the EMRI of a single BH around a supermassive one (see Section~\ref{sec:EMRI}), which are among the main targets of LISA.
For such configurations, the presence of a Galileon field could be hoped to be detected.


